Applications and Challenges of Fairness APIs in Machine Learning Software

Machine Learning software systems are frequently used in our day-to-day lives. Some of these systems are used in various sensitive environments to make life-changing decisions. Therefore, it is crucial to ensure that these AI/ML systems do not make any discriminatory decisions for any specific groups or populations. In that vein, different bias detection and mitigation open-source software libraries (aka API libraries) are being developed and used. In this paper, we conduct a qualitative study to understand in what scenarios these open-source fairness APIs are used in the wild, how they are used, and what challenges the developers of these APIs face while developing and adopting these libraries. We have analyzed 204 GitHub repositories (from a list of 1885 candidate repositories) which used 13 APIs that are developed to address bias in ML software. We found that these APIs are used for two primary purposes (i.e., learning and solving real-world problems), targeting 17 unique use-cases. Our study suggests that developers are not well-versed in bias detection and mitigation; they face lots of troubleshooting issues, and frequently ask for opinions and resources. Our findings can be instrumental for future bias-related software engineering research, and for guiding educators in developing more state-of-the-art curricula.

==> studyresults.tex <==
\section{Study Results}
In this section, we report a study that we conducted to understand the applications of 11 fairness API libraries in open-source ML software and the challenges 
of developing the 11 API libraries. The 11 API libraries are introduced in \sec\ref{sec:selection-apis}. 
 We answer four research questions (RQ):
\begin{enumerate}[label=\bf{RQ\arabic{*}}., leftmargin=30pt]
  \item \rev{What use cases the fairness API libraries are applied for in the open-source Machine Learning Software Applications (MLSAs)?} (see \sec\ref{sec:lib_usecases})
  \item How are the biases detected in these
  use-cases? (see \sec\ref{sec:rq-bias-detection-strategies}) 
  \item How are the biases mitigated in these use-cases? (see \sec\ref{sec:rq-bias-mitigation-strategies})
  % \item What challenges do the users of the API libraries face?
   \item What are the topics found in the issues that developers reported while using the API libraries? (see \sec\ref{sec:challenges-bias-apis})
\end{enumerate} The first three research questions (RQ1 - RQ3) aims to understand the application of the 11 fairness API libraries in real-world open-source ML software repositories. 
The last research question (RQ4) aims to investigate the challenges the developers of the 11 API libraries face while developing the API libraries. 

\subsection{RQ1. \rev{What use cases the fairness API libraries are applied for in the open-source Machine Learning Software Applications (MLSAs)?}}
\label{sec:lib_usecases}
\subsubsection{Motivation} Previous research has shown concerns about the possibility of bias in different types of ML models:
models for recruiting systems \cite{AmazonScrapsSecret}, for loan and credit approval systems \cite{chenFairLendingNeeds2018}, and for health care systems \cite{vokingerMitigatingBiasMachine2021}. 
In this research question, we investigate this issue in more detail by finding the distribution of use-cases, domains, and activities that deal with bias. 
\subsubsection{Approach}
%\subsubsection{Approach}
To find the use cases of the fairness API libraries, we label each of the selected 230
software repositories based on their intended actions. For this labeling, we
applied an open card sorting approach \cite{williamCardSorting2013}. The first
two authors (a graduate student, and a postdoc) worked together during the
labeling phase. These two authors synchronously communicated using Skype and
Zoom meetings. They have discussed the name, description, and README.md file of
each repository from GitHub using GitHub APIs.
In a few cases, specifically, when the projects are developed for tutoring
purposes, the intended use-cases were not clear from the metadata.
The two authors went through the source files of the repositories to find out
the intended use-cases.
More specifically, they have used project reports or documentation files, the
used fairness datasets, and APIs, the comments found within the driver file, and
the source code fragments where the bias-related APIs were used. 
% For example, the GitHub repo \href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML}  uses the Fairlearn API to integrate the auditing of fairness constraints during the development of an ML model within an AutoML pipeline. We thus label the use case as `Development'. 

%%%%%%%%%% Rev 1 %%%%%%%%
\rev{
For example, the GitHub repo \href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML} 
has been labeled as `ML Development Framework' use-case. The purpose of the auto ML framework is to 
develop a machine-learning pipeline using different automatic techniques. The 
repository \href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML} has added components to apply 
fairness constraints while developing different ML models. However, to test its generated pipeline using fairness 
constraints it used multiple fairness benchmark datasets from different domains (such as business, and health). 
As such, we see datasets from different domains even though the primary target of the repository is to develop a 
machine-learning model using an automated approach. This is why we labeled this repository under the `ML Development Framework' use-case.}

Similarly, another GitHub repo \href{https://github.com/dssg/hiv-retention-public}{dssg/hiv-retention-public} uses the Aequitas fairness 
API to detect bias in customer retention in clinical trials. We thus label the use case as `Patient Retention'.
Overall, the labeling of the uses took the two authors $\sim$25 hours in total. Although the plan was
to invite the third author (a professor) in case of disagreements, the intended
use-cases were so obvious that the third author did not have to involve. In the
end, the 230 repositories were labeled with 25 unique use-cases.

A use case scenario can be implemented by focusing on the implementation of a `service' using a fairness API or the 
incorporation into the ML system of a model-related feature offered by the fairness API.  
As such, in the second stage of our use case labeling process, we aimed to group the identified use cases 
into the domains for which they were implemented for. 
For example, we assign the use case `Patient Retention' to the `Service` domain, because it is about the implementation 
of a health-related service.  
%The output from this second stage is a list of domain names under which we could group each of the identified use cases. 
%For example, the use-cases named ``patient retention'', and ``disease prediction''  were merged into the
%higher-level ``Service'' domain.
% Similarly, ``credit approval'' and ``advertisement strategy'' use-cases were merged into the ``business'' domain. 
Similarly, ``Language Analysis'' and ``Recommendation'' user-cases were merged into the ``Model'' domain as these use-cases primarily used/targeted ML-based models. 
All the first three authors participated in this grouping process, which was completed after several iterations. 


A fairness API can be used to detect and/or mitigate biases. 
During the grouping of the use cases by their domains, we observed that such usage of the fairness APIs can belong to certain activity types. 
For example, the `Patient Retention' use case is about the prediction of patients that should/should not be retained by identifying and/or removing 
bias during the selection process. Therefore, we label the activity type for this use case as `Prediction'.  
Similarly, another use case `ML Development Framework' (as explained above) belongs to the activity type `Operation', given it is about the operationalization 
of an ML model by incorporating fairness constraints into the model development pipeline.
In total, the third author worked
$\sim$10 hours with the first two authors for these two levels of
categorization.

%\gias{here only discuss the results of RQ1, while moving the approach to the study setup section above}

% \gias{suggest the following flow for this RQ in order: \begin{enumerate}
%   \item show two pie charts side by side one for overall activity distribution and one for overall domain distribution. 
%   \item introduce and explain the activity and domain types in two paragraphs.
%   \item Then say we found total 30 use cases across the activity and domain types, and show their overall distribution like Fig. 3 from \url{https://rdcu.be/cxhHV}
%   \item Then say we group the use cases by the activity and domain types in a taxonomy and then say we explain 
%   the use cases by following taxonomy as follows. Now follow the presentation 
%   format of RQ1 from Section 4.1.3 \url{https://rdcu.be/cxhHV} (starting from page 16) - when you introduce a use case explain how the 
%   use case is implemented in a GitHub repo. You don't have to explain each use case with an example, 
%   only the most frequent one/two under each domain-activity pair combo
%   \item Now conclude by showing how the creation of the use cases (activity, domain) types evolved over time in the dataset. show two line charts, one for activity type and one for domain type.
% \end{enumerate}}



% \begin{figure}[t]
% % \subfloat[By activity types]
% %       {
% %       \centering\begin{tikzpicture}[scale=0.40]-
% %       \tikzstyle{every node}=[font=\footnotesize]
% %     \pie[
% %         /tikz/every pin/.style={align=center},
% %         text=pin, number in legend,
% %         explode=0.0, rotate=0,
% %          color={black!0, black!20, black!40, black!60},
% %         ]
% %         {
% %             50/\bf{Learning} (50\%),
% %             50/\bf{Non-Learning} (50\%)
% %         }
% %     \end{tikzpicture}
% %     \label{fig:usecase_activity_dist}
% %       }
% % \subfloat[By non-learning activity types]
% %       {
% %       \centering\begin{tikzpicture}[scale=0.40]-
% %       \tikzstyle{every node}=[font=\footnotesize]
% %     \pie[
% %         /tikz/every pin/.style={align=center},
% %         text=pin, number in legend,
% %         explode=0.0, rotate=45,
% %          color={black!0, black!20, black!40, black!60},
% %         ]
% %         {
% %             46/\bf{Prediction} (46\%),
% %             43.4/\bf{Analysis} (43.4\%),
% %             10.4/\bf{Operation} (10.4\%)
% %         }
% %     \end{tikzpicture}
% %     \label{fig:usecase_activity_dist_nonlearning}
% %       } \\
% \subfloat [By domains]
%       {
%       \centering\begin{tikzpicture}[scale=0.40]-
%       \tikzstyle{every node}=[font=\footnotesize]
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0, rotate=0,
%          color={black!0, black!20, black!40, black!60, black!80},
%         ]
%         {
%             63.5/\bf{Generic} (63.5\%),
%             36.5/\bf{Non-generic} (36.5\%)
%         }
%     \end{tikzpicture}
%     \label{fig:usecase_domain_dist}
%       } 
% \subfloat [By non-generic domains]
%       {
%       \centering\begin{tikzpicture}[scale=0.40]-
%       \tikzstyle{every node}=[font=\footnotesize]
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0, rotate=0,
%          color={black!0, black!20, black!40, black!60, black!80},
%         ] % [37.0, 24.9, 19.2, 13.2, 5.8]
%         {
%             % 37/\bf{Model} (37\%),
%             % 44.1/\bf{Business} (44.1\%),
%             % 13.2/\bf{Legal} (13.2\%),
%             % 5.8/\bf{Health} (5.8\%)
%             %%%
%             37/\bf{Model} (37\%),
%             63/\bf{Service} (63\%)
%         }
%     \end{tikzpicture}
%     \label{fig:usecase_domain_dist_nongeneric}
%       } 
%       \caption{\rev{Distribution of use-cases of the repositories}}
% \vspace{-3mm}
% \label{fig:usecase-dist}    
% \end{figure}

\begin{figure}[!thb]
\centering
\includegraphics[scale=.65]{figs/analysis/BiasUseCasesMod.pdf}
\caption{Taxonomy of the bias-related use-cases in the open source ML software systems that apply bias detection and/or mitigation APIs. 
Some of the use-cases (e.g., monitoring service) are shown multiple times because those are found under multiple activities.}
\label{fig:usecase_category_all}
%\vspace{-.5cm}
\end{figure}

\subsubsection{Results} 
\rev{We observed total of 25 distinct use cases in our 230 studied GitHub ML software repositories related to the usage of the 11 fairness API libraries. 
In \fig\ref{fig:usecase_category_all}, we categorize the 25 use cases in a taxonomy, where the 25 use cases belong to four types of activities: \begin{inparaenum}
\item Generic learning and exploration,
\item Non-generic use cases, such as: \begin{inparaenum}
\item Prediction,
\item Analysis, and 
\item Exploration.
\end{inparaenum}
\end{inparaenum} Each activity type can further be divided into two sub-types: \begin{inparaenum}
\item Model, and 
\item Service.
\end{inparaenum} We denote the activity sub-types as domains in the rest of this paper. To note, here we consider mitigation exploration and mitigation service as one distinct use case as both target the mitigation use case. Same applies for the detection exploration and detection service.
}
\begin{figure}[t]
\centering
\includegraphics[scale=.55]{figs/analysis/unique_usecase_percentage_horizontal_filtered.pdf}
\caption{\rev{Distribution of use cases by the total number of repositories considering only non-generic repositories.}}
\label{fig:usecase_percentage_filtered}
\end{figure}

\rev{
The generic-type use cases contain projects (63.5\% of all repositories), whose focus is mainly to create tutorials to support the learning 
of a bias API model or the implementation of a toy service using the bias APIs.  
For example, there are projects that implement different bias detection and mitigation 
algorithms (\href{https://github.com/andrijaster/FAIR}{andrijaster/FAIR}). These approaches are not focused on any 
specific domain and can be applied in various areas. The primary objective found in such repositories is to provide learning/educational materials.
As such, the generic type use cases mostly are implemented in notebooks, unlike the non-generic use cases (see below). 
The top part of \fig\ref{fig:usecase_category_all} summarizes the taxonomy of the 6 unique
use-cases that can be found on repositories that targeted the Generic domain,
including repositories that focused on educational materials and learning
activities. Among the two most frequently observed use cases under this category is \emph{Educational Materials}, which are projects that provide API
Documentation of fairness-related libraries and frameworks, and provide
tutorials on how to use these APIs. For example,
\href{https://github.com/Repoanonymous/Fairness_Metrics}{Repoanonymous/Fairness\_Metrics}
contains tutorials on how to use various fairness metrics using different
datasets.
The bottom part of \fig\ref{fig:usecase_category_all}
summarizes the taxonomy of the use-cases of the rest of the repositories that
focused on non-generic use-cases. The non-generic type use cases are found in the 36.5\% of the ML software repositories. These software repositories 
utilized the fairness APIs for actual real-world tasks.
\fig\ref{fig:usecase_percentage_filtered} shows the distribution of use-cases
focusing on the filtered set of non-generic repositories. For this repository
set, we find that the use cases `Monitoring Service' and `Credit Approval' are
the most frequent use cases. We discuss below the non-generic use cases by explaining the activity and domain types and use cases in detail.
}
%We now describe the activity types, domain types, and use-cases in more depth.

%three domains and three activity types.
% \ajoy{
% \begin{itemize}
% \item Describe that we removed learning and generic from rest of the analysis and mention how many repositories are found after filtering
% \end{itemize}
% }

% \fig\ref{fig:usecase_activity_dist} shows that we can classify the repositories into two top-level activity types: learning-focused activities and other non-learning-focused activities. Both Learning and Non-learning-based repositories have equal coverage of repository use-cases (50\% of repositories each). Now in \fig\ref{fig:usecase_activity_dist_nonlearning} we show the distribution of repositories if we further sub-divide Non-learning-based repositories into Analysis, Operation, and Prediction activities. Among these activities, Prediction activity can be found in the highest number of non-learning-focused repositories (46\% repositories), then Analysis (43.4\% repositories), and finally by Operation (10.4\% repositories).

%\fig\ref{fig:usecase_domain_dist} shows that we can classify the repositories into two top-level domains: repositories that focus on generic use-case domain and repositories that focus on more specific non-generic use-case domains. The number of repositories that focuses on the Generic domain (63.5 \% of all repositories) is greater in number than the non-generic ones. Now in \fig\ref{fig:usecase_domain_dist_nongeneric} we show the distribution of repositories if we further sub-divide Non-generic repositories into Model and Service domains. Among these domains, the service domain can be found in the highest number of non-generic repositories (63\% repositories), followed by Model (37\% repositories).

% \fig\ref{fig:usecase_activity_dist} shows the distribution of repositories according to the four top-level activity types: Learning, Analysis, Operation, and Prediction. , followed by Prediction (23\% repositories), then Analysis (21.7\% repositories), and finally by Operation (5.2\% repositories).
% \fig\ref{fig:usecase_domain_dist} shows the distribution of repositories according to the six domains: Generic, Model, Service, Business, Legal, and Health. Among these domains, Generic contains the highest number of repositories (63.5 \% of all repositories), followed by Model (13.5 \%).

% \fig\ref{fig:usecase_percentage} shows the distribution of the 25 use-cases. The use-cases are shown in decreasing order. The use-cases related to learning general API usage using Educational Materials (23.9\% of the repositories) and mitigation approaches (23.9\% of the repositories) are most common. Similarly 
 

% \fig\ref{fig:usecase_category} summarizes the taxonomy of the 25 unique use-cases, grouped together with their six higher-level domains and the four highest level activity types.



% \begin{figure}[t]
% \centering
% \includegraphics[scale=.6]{figs/analysis/unique_usecase_percentage_horizontal.pdf}
% \caption{Distribution of usecases by total number of repositories considering all 230 repositories.}
% \label{fig:usecase_percentage}
% \end{figure}


 


% \begin{figure}[t]
% \centering
% \includegraphics[scale=.58]{figs/analysis/usecase_categ_generic.pdf}
% \caption{Taxonomy of the generic use-cases that apply bias detection and/or mitigation APIs.}
% \label{fig:usecase_category_generic}
% %\vspace{-.5cm}
% \end{figure}
% 
% \begin{figure}[t]
% \centering
% \includegraphics[scale=.58]{figs/analysis/usecase_categ_nongeneric.pdf}
% \caption{Taxonomy of the non-generic use-cases that apply bias detection and/or mitigation APIs. For readability, some of the use-cases (e.g., monitoring service) are shown multiple times, because the same use-case can be under different domains and activities.}
% \label{fig:usecase_category_nongeneric}
% %\vspace{-.5cm}
% \end{figure}



% \rev{
% The \emph{Learning}, the largest activity type (50\%), contains projects that focus on providing learning resources in order to detect and mitigate bias in a system. It contains demo/tutorial projects showing bias API usage, in addition to projects that share any new approaches to identify or mitigate bias. For example, the project  \href{https://github.com/ckadner/ffdl-wsk-pipeline-demo}{ckadner/ffdl-wsk-pipeline-demo} provides a tutorial on how to integrate bias detection mechanism within a distributed serverless cloud platform (OpenWhisk).
% }


\nd\bf{$\bullet$ The three primary activity types found in non-generic repositories are \begin{inparaenum}[(1)]
\item Prediction, 
\item Analysis, and 
\item Operation.
\end{inparaenum}}

\begin{inparaenum}[(1)]
\item The \emph{Prediction} category contains projects (22.6\%) that are focused on prediction tasks.
For example, the project \href{https://github.com/satejsoman/chicago-business-viability}{satejsoman/chicago-business-viability} used bias detection APIs to identify bias in a business failure prediction task, and therefore enlisted under this category. A total of 18 different use-cases belong to this category. This category is so diverse that it contains all six relevant domains.

\item The \emph{Analysis} category contains projects (8.7\%) that analyze data and ML models. For example, the project \href{https://github.com/gunnaja/ml_fairness_tradeoffs}{gunnaja/ml\_fairness\_tradeoffs} compares how the performance (eg, accuracy) of a model varies before and after applying the bias mitigation approach. This type of analysis is important for analyzing the trade-offs between performance and fairness because imposing fairness
can often harm performance, such as accuracy in prediction \cite{menonCostFairnessBinary2018,chenWhyMyClassifier2018,zhaoInherentTradeoffsLearning2022}.

\item The \emph{Operation} category is the least prevalent and contains projects (5.2\%) that provide support during ML system operation. These activities were mainly focused on the development of ML models (i.e., \href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML}), and the deployment (i.e., \href{https://github.com/IBM/Trusted-ML-Pipelines}{IBM/Trusted-ML-Pipelines}) of the developed models. 

\end{inparaenum}


\nd\rev{\bf{$\bullet$ The two types of domains under a non-generic activity type are \begin{inparaenum}[(1)]
%\item Generic
\item Model and
\item Service.
% \item Business,
% \item Legal, and 
% \item Health.
\end{inparaenum}}
The \emph{Service} domain contains projects (63\% of non-generic repositories) that provide services, including flight cancellation, policy violation, 
and traffic handling. For example, the project \href{https://github.com/AnaTorresR/DPA-food_inspections}{AnaTorresR/DPA-food\_inspections} explores 
fairness within the process of restaurant inspection service of a city.  
If we dig deeper into this domain, we see repositories providing services in various types of use-cases. Some of such use-cases types are as follows:
\begin{inparaenum}[(i)]
    % (44.1\%)
    \item Business: These use-cases contain projects that provide support to business and financial needs, such as deciding about credit approval, predicting financial solvency, and developing advertisement strategies. For example, the project \href{https://github.com/kratikanaskulwar/Mitacs-Verafin-Internship}{kratikanaskulwar/Mitacs-Verafin-Internship} audits bias in fraud detection machine learning model's prediction. 
    % (13.2\%)
    \item Legal: Thesis use-cases contain projects that are related to legal rules, regulations, and law enforcement. Sometimes legal matters can be discriminatory towards certain groups of people. For example, the project \href{https://github.com/Caramel96/AIF360_Bias_Mitigation-police-stop-and-search-project}{Caramel96/AIF360\_Bias\_Mitigation-police-stop-and-search-project} explores discrimination in police stop and search strategy based on the race of an involved person.
    % (5.8\%)
    \item Health: These use-cases contain projects that are related to both physical and mental health. For example, the project  \href{https://github.com/drskaf/EHR-Prediction-Model-with-Tensorflow}{drskaf/EHR-Prediction-Model-with-Tensorflow} explores demography-based bias in calculating expected hospitalization time.
\end{inparaenum}
% %\item 
% (3) The \emph{Business} domain contains projects (44.1\%) that provide support to business and financial needs, such as deciding about credit approval, predicting financial solvency, and developing advertisement strategies. For example, the project \href{https://github.com/kratikanaskulwar/Mitacs-Verafin-Internship}{kratikanaskulwar/Mitacs-Verafin-Internship} audits bias in fraud detection machine learning model's prediction. This domain can also contain service as a business. For example, the project \href{https://github.com/AnaTorresR/DPA-food_inspections}{AnaTorresR/DPA-food\_inspections} explores fairness within the process of restaurant inspection service of a city. 
% %\item 
% (4) The \emph{Legal} domain contains projects (13.2\%) that are related to legal rules, regulations, and law enforcement. Sometimes legal matters can be discriminatory towards certain groups of people. For example, the project \href{https://github.com/Caramel96/AIF360_Bias_Mitigation-police-stop-and-search-project}{Caramel96/AIF360\_Bias\_Mitigation-police-stop-and-search-project} explores discrimination in police stop and search strategy based on the race of an involved person.
% %\item 
% (5) The \emph{Health} domain contains projects (5.8\%) that are related to both physical and mental health. For example, the project  \href{https://github.com/drskaf/EHR-Prediction-Model-with-Tensorflow}{drskaf/EHR-Prediction-Model-with-Tensorflow} explores demography based bias in calculating expected hospitalization time.
% %\end{inparaenum}
The \emph{Model} domain contains projects (37\% of non-generic repositories) that are directly related to the development, deployment, analysis, monitoring, and testing of ML models. For example, \href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML} develops models automatically using a low-code development strategy and checks bias in the developed model.
}

\nd\bf{$\bullet$  Out of the 25 use-cases 21 use cases belong to the non-generic activity types}.

Our replication package describes all of the use-cases that we show in \fig\ref{fig:usecase_category_all}. 
To provide insights about our findings, we discuss below several selected non-generic use-cases, covering all two domains, and the three different activities (i.e., Prediction, Analysis, and Operation). 

\begin{inparaenum}[(1)]
\item \emph{Monitoring (Service + Analysis)}: This use-case is related to projects
that focus on the analysis of System/API monitoring services. For example, for
specific datasets and prediction problems the application project,
\href{https://github.com/nirdizati-research/predict-python}{nirdizati-research/predict-python},
provides support to experienced users in finding the most suitable
predictive models.

% Generic + Learning


% Model + Operation
\item \emph{\rev{ML Development framework} (Model + Operation)} are projects related to developing a
pipeline for automated model development, checking bias while using AutoML tools
to develop models, neural network training, and certification. The project
\href{https://github.com/SotArchontas/AutoML}{SotArchontas/AutoML} falls into
this category because it is a project which integrates auditing of fairness
within the pipeline of AutoML-based low-code model development strategy.

% Business + Prediction
\item \emph{Insolvency Prediction (Service + Prediction)} are projects that,
given a customer profile, can predict financial insolvency (e.g., 
\href{https://github.com/arguz95/Project\_ML2}{arguz95/Project\_ML2}).

% Health + Prediction
\item \emph{Patient Retention (Service + Prediction)} are projects that predict
patient's retention in clinical care (e.g.,
\href{https://github.com/dssg/hiv-retention-public}{dssg/hiv-retention-public}).

% Legal + Prediction
\item \emph{Risk Detection (Service + Prediction)} are the projects that predict risk
of recidivism, and risk of corruption in the public procurement process (e.g., 
\href{https://github.com/alan-turing-institute/DSSG19-DNCP-PUBLIC}{alan-turing-institute/DSSG19-DNCP-PUBLIC}).


\end{inparaenum}

% Business + Analysis



\begin{figure}
% \subfloat[By activity type]
%       {
%       \centering
%       \includegraphics[scale=.55]{figs/analysis/usecase-activity-trends.pdf}
%       \label{fig:usecase-activity-trends}
%       } 
\subfloat [By generic vs non-generic activity types]
      {
      \centering
      \includegraphics[scale=.55]{figs/analysis/usecase-domain-trends.pdf}
      \label{fig:usecase-domain-trends}
      }  
% \\
% \subfloat[By non-learning activity type]
%       {
%       \centering
%       \includegraphics[scale=.55]{figs/analysis/usecase-activity-trends-nonlearning.pdf}
%       \label{fig:usecase-activity-trends-nonlearning}
%       } 
\subfloat [By domain types under the non-generic use cases]
      {
      \centering
      \includegraphics[scale=.55]{figs/analysis/usecase-domain-trends-nongeneric.pdf}
      \label{fig:usecase-domain-trends-nongeneric}
      }  \\      
      \caption{The evolution of the domain and activity types of the identified use cases based on the creation of the corresponding GitHub repositories.}
\vspace{-3mm}
\label{fig:usecase-trends}    
\end{figure}

\rev{
\fig\ref{fig:usecase-trends} provides insights into how these fairness-related repositories are growing over time. 
% \fig\ref{fig:usecase-activity-trends} shows that both learning-based and non-learning-based repositories are indeed increasing following a trend similar to one another.
% Moreover, \fig\ref{fig:usecase-activity-trends-nonlearning} suggests that in all the activity types, except Operation, the number of repositories is increasing significantly. 
% This growing trend is generally true in \fig\ref{fig:usecase-domain-trends} and \fig\ref{fig:usecase-domain-trends-nongeneric} as well; 
\fig\ref{fig:usecase-domain-trends} shows that both generic and non-generic repositories are indeed increasing and we see a more consistent growth trend for the non-generic repositories. Moreover, \fig\ref{fig:usecase-domain-trends-nongeneric} suggests that in both of the non-generic domains, the number of repositories is increasing significantly and the growth trend in service use-cases is more rapid. 
This observation implies the growing demand for bias detection and mitigation in machine learning software. We also observe that the Generic domain has the highest growth over time. This indicates that as fairness improvement is a newly emerging field, there is a growing need for education and learning materials. As a result, academics and API library developers should invest more time in developing more education and learning materials about fairness in machine learning software.
% This is a clear indication of the struggle of ML developers while dealing with fairness libraries (RQ4 discusses this in more detail).  
}

% created within a specific year increased over time (from 2017 to 2021). However, the lines dropped significantly for 2022 that's because we don't have the complete data for the whole year of 2022. 
% We see similar trends for domain types as well (in \fig\ref{fig:usecase-domain-trends}.  These trends signify that ML developers are increasingly using bias detection and mitigation APIs across different activity and domain types.


\begin{rqbox}{RQ1 Summary} 
The use-cases of bias detection and mitigation APIs are diverse. In our small,
but carefully curated, dataset of 230 projects, we found 25 unique use-cases
that belong to two different domains and four different activities. Among the observed use cases, some are 
related to various types of services (e.g., health, legal, and business), and others are related to the model-related operations from the fairness APIs (e.g., ML model deployment).
Our results show developers/users devote significant effort to learning the usage of fairness APIs (observed via the over 63\% generic use cases) 
At the same time, we observe that the usage of fairness APIs for real-world non-generic use cases is growing.
% We see upward trends of new repositories across different activity and domain types over time.
\end{rqbox}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RQ2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{RQ2. How are the biases detected in the use-cases?}\label{sec:rq-bias-detection-strategies}
%\subsubsection{Approach}
%We present this classification in \fig\ref{fig:detection_approaches}.

%\subsubsection{Results}
% There exists two main source of bias within an ML system: data and the predictions. So, the bias detection metrics can be classified into two higher level categories:
% \begin{inparaenum}[(1)]
% \item Dataset metrics: These metrics computes bias in the dataset; 
% \item Model prediction metrics: These metrics computes bias in the prediction of the ML models outcome.
% \end{inparaenum}

% Moreover we can also divide t
% \begin{inparaenum}[(1)]
% \item Group fairness metrics:
% \item Individual fairness metrics:
% \end{inparaenum}

% \begin{figure}[htb]
% \centering
% \includegraphics[scale=.6]{figs/analysis/detection_approaches.pdf}
% \caption{Classification of bias detection metrics \shaiful{In the figure highlight the portion that was not in Castelnovoa et al.'s classification.} \ajoy{updated}}
% \label{fig:detection_approaches}
% \end{figure}


% We see in \fig\ref{fig:detection_approaches} that group fairness metrics (57\% of all detected metrics) and generic metrics (41.4 \% of all detected metrics) are the most used fairness metrics in our repository dataset followed by those fairness metrics that can be applied to calculate both group and individual fairness (Group-Individual metrics, 1.6 \% of all detected metrics).

% \begin{figure}
% \centering
% \subfloat
%       {
%       \centering\begin{tikzpicture}[scale=0.50]-
%       \tikzstyle{every node}=[font=\footnotesize]
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0, rotate=45,
%          color={black!10, black!30, black!50, black!70},
%         ]
%         {
%             57/\bf{Group fairness metrics} (57\%),
%             1.6/\bf{Group-Individual fairness metrics} (1.6\%),
%             41.4/\bf{Utility fairness metrics} (41.4\%)
%         }
%     \end{tikzpicture}
%       } 
% \caption{Distribution of the used fairness metrics}
% \vspace{-3mm}
% \label{fig:detection_dist}    
% \end{figure}

% \begin{table*}[htbp]

%   %\def\arraystretch{1.5}
%     \centering

    
%     \caption{Usage of bias detection metrics in different use-cases\gias{under the use-cases column, let's show a bar line with distrubition of domain types like Table VII from here \url{https://arxiv.org/pdf/2201.04241.pdf}. Leave the mention of the specific use case names for textual description and not for this table}}
    
%     \label{tab:detection_usecases}
%     \scalebox{0.8}{
%     \begin{tabular}{llllr}
%     \toprule
%     \textbf{Metrics}  	&  \textbf{Metrics}  &		 \textbf{Use-case}  &			 \textbf{Use-cases}  &  \textbf{Repository}\\
%     \textbf{Category}  	&  \textbf{Sub-Category}  &		 \textbf{Category}  &			 						&	 \textbf{Count} \\ \midrule
% Generic &   & Learning & Generic (Mitigation, Detection, API Usage) & 90 \\
%  &  & Prediction & Service (Policy Violation, Traffic Handler, Monitoring, Flight Cancellation), \\
%  &  &   &   Legal (Risk Detection, Action Prediction), Generic (Survivability Prediction), \\
%  &  &   &   Health (Disease Prediction, Patient Retention), Business (Advertisement Strategy,  \\
%  &  &   &   Fraud Detection, Failure Prediction, Credit Approval, Insolvency Prediction, \\
%  &  &   &   Monetary Compensation), Model (Recommendation) & 48 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring), Service (Detection, Monitoring), \\
%  &  &   &   Model (Model Security, Language Analysis, Monitoring) & 43 \\
%  &  & Operation & Model (Deployment, Development) & 9 \\
% \cline {2-5}
% \cline {1-5}
% Group & Separation & Learning & Generic (Mitigation, Detection, API Usage) & 28 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring), Model (Model Security, Monitoring), \\
%  &  &   &   Service (Detection) & 10 \\
%  &  & Prediction & Generic (Survivability Prediction), Health (Disease Prediction), \\
%  &  &   &   Business (Credit Approval), Legal (Risk Detection, Legal Status Prediction) & 5 \\
%  &  & Operation & Model (Deployment, Development) & 4 \\
% \cline {2-5}
%  & Independence & Learning & Generic (Mitigation, Detection, API Usage) & 25 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring), Model (Model Security, Monitoring) & 9 \\
%  &  & Operation & Model (Deployment, Development) & 5 \\
%  &  & Prediction & Legal (Legal Status Prediction) & 1 \\
% \cline {2-5}
%  & Sufficiency & Learning & Generic (Mitigation, Detection, API Usage) & 12 \\
%  &  & Analysis & Generic (Monitoring) & 1 \\
%  &  & Operation & Model (Development) & 1 \\
% \cline {2-5}
% \cline {1-5}
% Group-Individual &  & Learning & Generic (Mitigation, API Usage) & 2 \\
% \cline {2-5}
% \cline {1-5}
% Subgroup &  & Learning & Generic (Mitigation, API Usage) & 2 \\
% \cline {2-5}
% \cline {1-5}
% Individual &  & Learning & Generic (Detection) & 1 \\
% \cline {2-5}
% \cline {1-5}

% \end{tabular}
% }
% \end{table*}


% \gias{suggest the following flow for this RQ:
% \begin{enumerate}
%   \item First show two pie charts side by side on the distribution of the detection strategies per use case activity type and domain type.
%  \item Then say the detection strategies can be grouped under five types: generic, group, individual, \ldots Then briefly explain in one paragraph what the five types mean and refer to an existing paper to the reader if he/she wants to learn about that in detail. 
%   \item Then say the five detection strategies are found across the GitHub repos (show the current Fig. 3) and explain in one single paragraph. 
%   \item Now say the use cases can be grouped under the five detection strategies as follows. Refer to current Table 2. 
%   \item Now explain one/two detection strategies with example per the five detection strategies by picking the most frequent/representative use case under it.
%   \item Now conclude by showing a line chart on the evolution (i.e., creation) of the five detection strategies in our dataset.
% \end{enumerate}
% }

\subsubsection{Motivation} Numerous bias detection metrics have been proposed by
the research community, and many of them have already been implemented. For
example, the AI Fairness 360 library has implemented about 70 types of fairness
metrics \cite{AIFairness3602018} as Python APIs. The objective of this research
question is to explore how the real-world software projects apply these
libraries for detecting bias across the use cases we identified in \sec\ref{sec:lib_usecases}.

\subsubsection{Approach}\label{sec:rq2-approach} In \sec\ref{sec:lib_usecases}, we found that around 36.5\% of the ML software 
repositories in our dataset contained use cases that are non-generic, i.e., the use cases are applied for real-world 
applications where bias and fairness concerns need to be addressed. Given the relative importance of those non-generic use cases over the 
generic use cases, in this research question we specifically focus on the bias detection approaches used in the non-generic use cases.
As such, we analyze 84 ML sofrware repositories that contiained the non-generic use cases.
 
Each GitHub repository in our  dataset for non-generic use cases has used at least one of the fairness API libraries
listed in Table~\ref{tab:libraries}. Each of these API libraries has
multiple methods. Each method can use one or more fairness metrics to detect bias. 
It is possible that a project in our final set did not
use all the available methods from a library. To understand how an API is used to detect bias in a given use case scenario, 
we first listed all the
available methods within our selected API libraries. For most API libraries, it was done by
studying their well-written documentation that listed all the available
detection and mitigation methods. For libraries without sufficient documentation,
we studied their publication sources (i.e., published research papers), GitHub
README files, and inspected the project's source code when necessary. 

\rev{
Before we were able to analyze how the available APIs are being used across the selected set of repositories, we first needed to collect all the API calls that had been done utilizing the library imports within our selected repositories. For this, we used AST analysis approach utilizing the AST module from Python standard library. During this AST analysis approach, we considered various possible ways of importing API libraries and performing the API/function calls. For example, we considered both globally scoped module imports as well as locally scoped imports, calling APIs using techniques other than direct API calls (e.g., assigning the API into an attribute and later using that attribute for API calls, etc). Considering such cases helped us to lessen the number of missed/undetected valid API calls. We then used the \textit{substring} matching approach to match the extracted method names from these selected software projects' source code against our prepared list of available APIs (here, detection methods). 
}

Once the methods are identified, we manually determine the fairness metrics that are used from the methods 
in a GitHub repo. We then find the usage of these metrics within our selected GitHub repositories.
Finally, we classify the bias detection metrics to understand their distribution across 
these repositories and the identified use cases. This classification primarily
focuses on the cardinality of the involved parties---i.e., whether we are
measuring fairness among population groups or individuals. 
The classification uses the five types of bias detection metrics we discussed in \sec\ref{sec:background-bias-detection}.

\rev{To note, it is possible that one repository used several types of bias detection or mitigation methods. For such cases, when we counted the number of repositories for a given detection or mitigation method, the same repository was counted separately for each of the methods (e.g., ~\fig\ref{fig:detection_metrics}).}

%\rev{
%To note, unless otherwise specified, for the rest of the analysis, we only considered repositories that focused on non-generic domains. We have 84 such repositories in our selected set of 230 repositories.
%}


\begin{figure}[t]
\subfloat[By activity types]
      {
      \centering\begin{tikzpicture}[scale=0.40]-
      \tikzstyle{every node}=[font=\footnotesize]
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=45,
         color={black!0, black!20, black!40, black!60},
        ]
        {
            % 49.3/\bf{Learning} (49.3\%),
            % 23.7/\bf{Analysis} (23.7\%),
            % 21.8/\bf{Prediction} (21.8\%),
            % 5.2/\bf{Operation} (5.2\%)
            %%%%
            25/\bf{Analysis} (25\%),
            61.25/\bf{Prediction} (61.3\%),
            13.75/\bf{Operation} (13.7\%)
        }
    \end{tikzpicture}
    \label{fig:detection_activity_dist}
      } 
\subfloat [By domains]
      {
      \centering\begin{tikzpicture}[scale=0.40]-
      \tikzstyle{every node}=[font=\footnotesize]
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=0,
         color={black!0, black!20, black!40, black!60, black!80, black!90},
        ]
        {
            % 62.1/\bf{Generic} (62.1\%),
            % 13.7/\bf{Model} (13.7\%),
            % 10/\bf{Service} (10\%),
            % 7.6/\bf{Business} (7.6\%),
            % 4.3/\bf{Legal} (4.3\%),
            % 2.4/\bf{Health} (2.4\%)
            %%%
            % 36.25/\bf{Model} (36.25\%),
            % 46.25/\bf{Business} (46.25\%),
            % 11.25/\bf{Legal} (11.25\%),
            % 6.25/\bf{Health} (6.25\%)
            %%%
            36.25/\bf{Model} (36.25\%),
            63.75/\bf{Service} (63.75\%)
        }
    \end{tikzpicture}
    \label{fig:detection_domain_dist}
      } 
      \caption{Distribution of the use-case domains of the repositories that used fairness metrics}
\vspace{-3mm}
\label{fig:detection-dist}    
\end{figure}


\begin{figure}[t]
\subfloat[By detection metrics type]
      {
      \centering\begin{tikzpicture}[scale=0.40]-
      \tikzstyle{every node}=[font=\footnotesize]
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=45,
         color={black!0, black!40},
        ]{
            82/\bf{Utility} (82\%),
            18/\bf{Non-utility} (18\%)
        }
    \end{tikzpicture}
    \label{fig:detection_metric_types}
      } \\
\subfloat [By non-utility metrics type]
      {
        \centering
        \includegraphics[scale=.4]{figs/analysis/detection_approaches_sunburst_edited_updated.pdf}
        % \caption{Classification of bias detection metrics.}
        \label{fig:detection_approaches}
      } 
      \caption{Distribution of the fairness metrics across all the 84 repositories that contained non-generic use cases.} 
\vspace{-3mm}
\label{fig:detection_metrics}    
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[scale=.5]{figs/analysis/detection_approaches_sunburst_edited_updated.pdf}
% \caption{Classification of bias detection metrics.}
% \label{fig:detection_approaches}
% \end{figure}

\subsubsection{Results}\label{sec:rq-bias-detection-results} 
\fig\ref{fig:detection_activity_dist} shows the distribution of the activity types that used bias detection APIs. 
Prediction (61.3\%) is the activity type that contains most of the used bias detection metrics, followed by Analysis, and finally by Operation. 

% This ranking follows the ranking of overall repository ranking from \fig\ref{fig:usecase_activity_dist}.
Figure~\ref{fig:detection_domain_dist} shows the distribution of the domains (from our dataset) that applied bias detection APIs. 
Consistent with our earlier findings (RQ1), service is the most dominant domain (63.75\%) of the two non-generic domains. 
However, Model also has a fair share (36.25\%) of the API usages. 

Figure~\ref{fig:detection_approaches} shows the distribution of the five bias
detection metric types across the selected 84 GitHub repos where the 11 fairness API libraries
are used (see \sec\ref{sec:background-bias-detection} for an overview of the
metric types).
Most of the projects (73.5\%) in our dataset detected bias with the adoption and
modification of the utility metrics. Group fairness metrics were directly
applied by 23.8\% of the projects. Other categories, such as bias detection for
subgroups and individuals are rare.

\rev{
Table~\ref{tab:detection_usecases} shows how these bias detection APIs have been
used across the use-cases we found in \sec\ref{sec:lib_usecases}. Here we reported the usage based on both unfiltered (all of 230 repositories) and filtered set of non-generic repositories as some of the detection APIs (i.e., Individual, Subgroup, and Group-Individual) were only been found within the Generic use-case-focused repositories. For each metric type, we mention how many of the generic and non-generic repositories contain usage of this metric and present the domain distribution of the non-generic repositories.
}
In Table~\ref{tab:detection_usecases}, we see that for all of the metric types, the number of repositories in the generic domain is higher than in the non-generic domains. Unsurprisingly, a large number of repositories (116 of the repositories) from the generic domain use utility metrics. However, we also see the usage of utility metrics in non-generic domains and activities.  
Moreover, we observe that group-individual, subgroup, and individual fairness metrics are used only in generic domains. This implies that sensitive domains such as health, legal, and business have not considered subgroup or individual fairness at all in our repository dataset.

% \begin{table}[t]
%   %\def\arraystretch{1.5}
%     \centering

%     \caption{Distribution of the bias detection metrics across the different use-cases in our studied GitHub repositories. \#R = number of GitHub repositories. 
%     Color bar denotes a domain type: G = Generic (Black), M = Model (Green), B = Business (Red), L = Legal (Blue), H = Health (Orange)} %S = Service (Magenta)
    
%     \label{tab:detection_usecases}
%     %\scalebox{0.8}{
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lll|l}
%     \toprule
%     \textbf{Metrics}  	&		 \textbf{Use-case}  &			\textbf{\#R} &   \textbf{\% Distribution of Repos by Use-case Domains} \\
%     \midrule
% Utility & Learning & 90 & \sixbars{100}{0}{0}{0}{0}{0} \\
%   & Prediction & 48 & \sixbars{3}{2}{0}{69}{16}{9} \\
%   & Analysis & 43 & \sixbars{70}{26}{0}{4}{0}{0} \\
%   & Operation & 9 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% Group & Learning & 28 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Separation & Analysis & 10 & \sixbars{67}{27}{0}{7}{0}{0} \\
%   & Prediction & 5 & \sixbars{33}{0}{0}{17}{33}{17} \\
%  & Operation & 4 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% Group & Learning & 25 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Independence  & Analysis & 9 & \sixbars{73}{27}{0}{0}{0}{0} \\
%  & Operation & 5 & \sixbars{0}{100}{0}{0}{0}{0} \\
%  & Prediction & 1 & \sixbars{0}{0}{0}{0}{100}{0} \\
% \cmidrule {2-4}
% Group & Learning & 12 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Sufficiency  & Analysis & 1 & \sixbars{100}{0}{0}{0}{0}{0} \\
%   & Operation & 1 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% Group-Individual & Learning & 2 & \sixbars{100}{0}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% Subgroup & Learning & 2 & \sixbars{100}{0}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% Individual & Learning & 1 & \sixbars{100}{0}{0}{0}{0}{0} \\
% \bottomrule
% \end{tabular}%
% %}
% \end{table}


\begin{table}[t]
  %\def\arraystretch{1.5}
    \centering

    \caption{Distribution of the bias detection metrics across the different use-cases in our studied GitHub repositories. \#R = number of GitHub repositories. 
    Color bar denotes a domain type: M = Model (Black) and S = Service (Green)} %S = Service (Magenta)
    
    \label{tab:detection_usecases}
    %\scalebox{0.8}{
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lll|l}
    \toprule
    \textbf{Metrics} 	&  \textbf{Non-generic Use-case}  &			\textbf{\#R} &   \textbf{\% Distribution of Repos by Use-case Domains} \\
    \midrule
\textit{Utility} & Prediction & 47 & \sixbars{2}{98} \\
Non-generic: 74 %Generic: 116  
& Analysis & 18 & \sixbars{88}{12} \\
 & Operation & 9 & \sixbars{100}{0} \\
\cmidrule {2-4}
\cmidrule {1-4}
\textbf{Group} &  &   &    \\
\textit{Separation}  & Analysis & 4 & \sixbars{80}{20} \\
Non-generic: 12%Generic: 35  
& Prediction & 4 & \sixbars{0}{100} \\
 & Operation & 4 & \sixbars{100}{0} \\
\cmidrule {2-4}
\textit{Independence}  & Operation & 5 & \sixbars{100}{0} \\
Non-generic: 9%Generic: 31  
& Analysis & 3 & \sixbars{100}{0} \\
 & Prediction & 1 & \sixbars{0}{100} \\
\cmidrule {2-4}
\textit{Sufficiency}  & Operation & 1 & \sixbars{100}{0} \\
%\multicolumn{4}{l}{%Generic: 13, 
%Non-generic: 1} \\
%\cmidrule {2-4}
%\cmidrule {1-4}
%\multicolumn{4}{l}{The following three metrics classes have only generic user cases}\\
%\multicolumn{4}{l}{Group-Individual: 2 generic use cases, Subgroup: 2, Individual: 1}\\
% \textit{Group-Individual} & \multicolumn{3}{c}{Generic: 2} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% \textit{Subgroup} & \multicolumn{3}{c}{Generic: 2} \\
% \cmidrule {2-4}
% \cmidrule {1-4}
% \textit{Individual} & \multicolumn{3}{c}{Generic: 1} \\
\bottomrule
\end{tabular}%
%}
\end{table}

In order to have more insights into how developers implement bias detection libraries, we provide two concrete examples of bias detection below. 

% \begin{lstlisting}[caption={Execute functor in given thread in QT - Answer id 21653558 in Stack Overflow, shows  vulnerability due to use malloc function without checking return special condition, (CWE-1006, CWE-252, CWE-789, CWE-476)},label={lst:vuln2},basicstyle=\footnotesize]
% class FunctorCallEvent: public QMetaCallEvent {
% public:
%   template <typename Functor>
%     FunctorCallEvent(Functor && fun, QObject * receiver) :
%       QMetaCallEvent(new QtPrivate::QFunctorSlotObject<Functor, 0, typename QtPrivate::List_Left<void, 0>::Value, void>
%              (std::forward<Functor>(fun)), receiver, 0, 0,0,(void**)<@\textcolor{black}{\colorbox{yellow}{\textbf{malloc}}@>(sizeof(void*)))};
% \end{lstlisting}


\textbf{\textit{Metropolitan police}}: This use-case is implemented in a GitHub repo
\href{https://github.com/danladishitu/CE888-7-SP}{danladishitu/CE888-7-SP}, 
where the developer wanted to find out if there is any bias based on
the ethnicity of a person when metropolitan police had to use force in certain
situations. The implementation involves the following steps:

\begin{inparaenum}[(1)]
\item Importing the relevant bias-related methods from the \texttt{aif360} API
(Listing \ref{lst:usecase1_import}).
\item Preparing the dataset for applying bias detection metrics or mitigation
algorithms (Listing \ref{lst:usecase1_dataset}). Here the developer used a
dataset with binary label and ethnicity as the protected attribute.
\item Detecting bias on the classifier's prediction (Listing
\ref{lst:usecase1_detection}). Here, all three kinds of group bias
detection metrics such as sufficiency (True positive rate, True negative rate),
separation (Average odd difference), and independence (Disparate impact) were
used to calculate group fairness in the classifier's output. In \sec\ref{sec:background-bias-detection}, we provided more details about these fairness metrics.
% \item Mitigating bias by applying bias mitigation algorithm (see, Listing \ref{lst:usecase1_mitigation}). Here we see that a popular pre-processing technique, Reweighing, has been used to mitigate bias. 
% After applying mitigation algorithm the developers generally verify whether the situation improved or not by re-calculating bias detection metrics. 
\end{inparaenum}

\begin{lstlisting}[caption={Use-case1: API imports},label={lst:usecase1_import},basicstyle=\footnotesize]
from aif360.datasets import BinaryLabelDataset 
from aif360.metrics import ClassificationMetric
from aif360.explainers import MetricTextExplainer  
from aif360.algorithms.preprocessing import Reweighing
\end{lstlisting}


\begin{lstlisting}[caption={Use-case1: Preparing dataset for applying the API},label={lst:usecase1_dataset},basicstyle=\footnotesize]
bld = <@\textcolor{black}{\colorbox{yellow}{BinaryLabelDataset}}@>(df=pd.concat((x, y_true),
            axis=1),
            label_names=['Impact Factor: Possesion of a weapon'],
            protected_attribute_names=['SubjectEthnicity'],
            favorable_label=1,
            unfavorable_label=0)
privileged_groups = [{'SubjectEthnicity': 1}]
<@\textcolor{black}{\colorbox{yellow}{unprivileged\_groups}}@> = [{'SubjectEthnicity': 0}]
\end{lstlisting}

\begin{lstlisting}[caption={Use-case1: Detecting bias using various classification metrics},label={lst:usecase1_detection},basicstyle=\footnotesize]
valid_metric =  <@\textcolor{black}{\colorbox{yellow}{ClassificationMetric}}@>(bld, bld_preds, 
            unprivileged_groups=unprivileged_groups,
            privileged_groups=privileged_groups)

balanced_accuracy.append(0.5 * (valid_metric. <@\textcolor{black}{\colorbox{yellow}{true\_positive\_rate}}@>()
            + valid_metric. <@\textcolor{black}{\colorbox{yellow}{true\_negative\_rate}}@>()))
avg_odd_diff.append(valid_metric. <@\textcolor{black}{\colorbox{yellow}{average\_odds\_difference}}@>())
disp_impact.append(np.abs(valid_metric. <@\textcolor{black}{\colorbox{yellow}{disparate\_impact}}@>() - 0.5))
\end{lstlisting}


\textbf{\textit{Hospitalization time}} use case is implemented in the GitHub repo 
\href{https://github.com/drskaf/EHR-Prediction-Model-with-Tensorflow}{drskaf/EHR-Prediction-Model-with-Tensorflow}. The primary 
aim of this project is to estimate hospitalization time of patients. In this prediction of hospitalization time, the developers also used demographic information (such as race and gender). So, in order to check whether the prediction of their trained model is biased towards any demography groups, the developer used group bias detection API from the Aequitas library. 
Their implementation is consist of three steps: 
\begin{inparaenum}[(a)]
\item Importing the appropriate APIs (Listing \ref{lst:usecase2_import}).
\item Calculating group fairness considering race and gender as sensitive attributes (Listing \ref{lst:usecase2_detail}).
\item Plotting the output of the fairness metrics for better understanding (Listing \ref{lst:usecase2_plotting}). 
\end{inparaenum}
%%%% Only detection example
\begin{lstlisting}[caption={Use-case2: API imports},label={lst:usecase2_import},basicstyle=\footnotesize]
from aequitas.preprocessing import preprocess_input_df
from aequitas.group import Group
from aequitas.plotting import Plot
from aequitas.bias import Bias
from aequitas.fairness import Fairness
\end{lstlisting}

\begin{lstlisting}[caption={Use-case2: Calculating and visualizing group fairness},label={lst:usecase2_detail},basicstyle=\footnotesize]
ae_subset_df = pred_test_df[['race', 'gender', 'score', 'label_value']]
ae_df, _ = <@\textcolor{black}{\colorbox{yellow}{preprocess\_input\_df}}@>(ae_subset_df)
g = Group()
xtab, _ = g.get_crosstabs(ae_df)
absolute_metrics = g.<@\textcolor{black}{\colorbox{yellow}{list\_absolute\_metrics}}@>(xtab)
clean_xtab = xtab.fillna(-1)
aqp = Plot()
b = Bias()

# Reference Group Selection
# test reference group with Caucasian Male
bdf = b.<@\textcolor{black}{\colorbox{yellow}{get\_disparity\_predefined\_groups}}@>(clean_xtab, 
                    original_df=ae_df, ref_groups_dict={'race':'Caucasian', 'gender':'Male'}, 
                    alpha=0.05, check_significance=False)

f = Fairness()
fdf = f.<@\textcolor{black}{\colorbox{yellow}{get\_group\_value\_fairness}}@>(bdf)
\end{lstlisting}

\begin{lstlisting}[caption={Use-case2: Plotting fairness metrics},label={lst:usecase2_plotting},basicstyle=\footnotesize]
# Race and Gender Bias Analysis for Patient Selection
# Plot two metrics

# Is there significant bias in your model for either race or gender?
p = aqp.<@\textcolor{black}{\colorbox{yellow}{plot\_group\_metric\_all}}@>(xtab, metrics=['tpr', 'ppr'], ncols=2)

# Fairness Analysis Example - Relative to a Reference Group
# Reference group fairness plot
fpr_disparity = aqp.<@\textcolor{black}{\colorbox{yellow}{plot\_disparity}}@>(bdf, group_metric='fpr_disparity', 
                                        attribute_name='race')
\end{lstlisting}

% The third use-case example (denoted as Use-case3) is a business domain project from \href{https://github.com/satejsoman/chicago-business-viability}{satejsoman/chicago-business-viability} repository where the repository owners wanted to find out the viability of doing business in Chicago. The developer used the fairness metric to check whether the trained prediction model is biased towards \# of previous license renewals of the business (see Listing \ref{lst:usecase2_detail}). 

% %%%% Only detection example
% \begin{lstlisting}[caption={Use-case3: API imports},label={lst:usecase3_import},basicstyle=\footnotesize]
% from aequitas.group import Group
% from aequitas.preprocessing import preprocess_input_df
% \end{lstlisting}

% \begin{lstlisting}[caption={Use-case3: Calculating and visualizing group fairness},label={lst:usecase3_detail},basicstyle=\footnotesize]
% df, cols = <@\textcolor{black}{\colorbox{yellow}{preprocess\_input\_df}}@>(df)

% g = Group()
% xtab, _ = g.get_crosstabs(df, attr_cols=["num_renewals"])
% print(xtab)
% absolute_metrics = g.<@\textcolor{black}{\colorbox{yellow}{list\_absolute\_metrics}}@>(xtab)
% print(xtab[[col for col in xtab.columns if col not in absolute_metrics]])
% \end{lstlisting}



% \begin{figure}
% \subfloat[By detection metrics type]
%       {
%       \centering
%       \includegraphics[scale=.55]{figs/analysis/detection-type-trends-utility.pdf}
%       \label{fig:detection-trends-utility}
%       } \\
% \subfloat [By non-utility metrics type]
%       {
%       \centering
%       \includegraphics[scale=.55]{figs/analysis/detection-type-trends-nonutility.pdf}
%       \label{fig:detection-trends-nonutility}
%       } \\  
%       \caption{Evolution of the bias detection metric categories based on the creation of the corresponding GitHub repositories.}
% \vspace{-3mm}
% \label{fig:detection-trends}    
% \end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.65\columnwidth,keepaspectratio]{figs/analysis/detection-type-trends-filtered.pdf}
\caption{Evolution of the bias detection metric categories based on the integration of the APIs on corresponding GitHub repositories.}
\vspace{-3mm}
\label{fig:detection-trends}
\end{figure}


\rev{
We are also interested to learn how the fairness metrics used in our selected repository
set evolved over time. To perform such trend analysis, we first collected the source code of all selected repositories along with the full git source tree. We needed the full git tree because we want to see which APIs from the available APIs (from our selected API libraries) had been used within a particular year. So, for each repository we considered one commit per year starting from the repository creation date, more specifically, we considered the last commit of each year as the final state of that repository in that year. After that, we performed the API detection steps (described in \sec\ref{sec:rq2-approach}) on those selected set of commits by checking out the source code of the repository at those selected set of commits individually. Finally, after performing these steps, we had a list of used detection APIs against each year of the repository development for each repository. We then used this information for performing the trend analysis that we describe below.
}

\fig\ref{fig:detection-trends} shows that the application
of the utility and group fairness metrics has increased over time. The adoption
of the utility metrics dropped in 2021. In contrast, the group fairness metrics
have been used monotonously after 2018; probably because the API users are
becoming more aware of the available fairness metrics and started to use metrics
that are specific to their needs. We didn't find any use of the other three fairness metrics within the filtered set of non-generic repositories.
% There was no growth for the other three fairness metrics.


\begin{rqbox}{RQ2 Summary} 
Although there are five categories of fairness metrics, all of the non-generic software repositories use only the utility or the group fairness metrics for bias detection. Fairness for subgroups and individuals has been largely ignored, which could be devastating in systems where bias may incur at finer levels. Future studies should explore the challenges of developing and adopting these finer-level bias detection metrics.
\end{rqbox}


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RQ3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{RQ3. How are the biases mitigated in these use-cases?}\label{sec:rq-bias-mitigation-strategies}
% \gias{suggest the following flow for this RQ:
% \begin{enumerate}
%   \item First show two pie charts side by side on the distribution of the mitigation strategies per use case activity type and domain type.
%   \item Then say the mitigation strategies can be grouped under three types: pre, in post, \ldots Then briefly explain in one paragraph what the three 
%   types mean and refer to an existing paper to the reader if he/she wants to learn about that in detail. 
%   \item Then say the three mitigation strategies are found across the GitHub repos (show the current Fig. 3) under 24 mitigation types and refer to the current taxonomy fig. 5. 
%   \item Then say the 24 mitigation types are taken from the literatue and they are summarized in current Table 3. Say for details of the mitigation types refer to an existing paper.
%   \item Now say, below we explain the mitigation types with examples based on their 3 mitigation strategies.
%   \item Now for each strategy, pick one/two most representative mitigation type with example and explain it.
%   \item Now say the migitation strategies are found across the use case types and refer to current Table 4. Briefly explain the table results in one paragraph. 
%   \item Now conclude by showing a line chart on the evolution (i.e., creation) of the mitigation strategies in our dataset.
% \end{enumerate}
% }


% After detecting all the APIs, we group these together based on their base mitigation approach/algorithm. In \tbl\ref{tab:mitigation_approach} we summarize these mitigation approaches. To understand which higher-level techniques these mitigation APIs generally use, we categorize our prepared list of all available mitigation approaches using a high-level categorization. Two of the authors went through the source materials of these mitigation approaches to prepare for this higher-level categorization. We present this categorization in \fig\ref{fig:mitigation_approach}.

\subsubsection{Motivation} Similar to the bias detection approaches, numerous bias mitigation approaches have been proposed and developed. 
The objective of this research question is to explore how real-world software projects apply these libraries for bias mitigation. 

\subsubsection{Approach}
Similar to RQ2, we focus on the 84 GitHub repositories that utilized the fairness APIs for 
non-generic use cases. Each GitHub repository in the final set has used at least one of the fairness API libraries
listed in Table~\ref{tab:libraries}. Seven out of the 11 API libraries offer methods to mitigate bias. Each of these API libraries has
multiple methods to mitigate the biases. It is possible that a project in our final set did not
use all the available methods from an API. We, therefore, first identify 
which mitigation methods of an API are used in each of our studied GitHub repos. 

Similar to our analysis of bias detection methods (discussed in \sec\ref{sec:rq2-approach}), 
we consulted the API documentation, GitHub README files, and corresponding publication sources 
to collect the names of mitigation methods in each API. We then used
the \textit{substring} approach to match the collected method names against the method names imported from the API in the 
source from of each GitHub repo. 

\tbl\ref{tab:mitigation_approach} shows the bias mitigation approaches that have
been implemented as APIs in our selected libraries. Most of these APIs (written
in \textit{italic}) have been published as research articles. A few of the
mitigation approaches (e.g., Correlation remover,  Upsampling) are, however,
provided out of the box by the libraries to mitigate bias. Evidently, AI
Fairness 360, and EthicML are the most prevalent; they have most of the
mitigation approaches implemented. On the contrary, other libraries have
implementation only for a few selected mitigation approaches.
For example, BlackBoxAuditing has implementation only for the disparate impact
remover approach. Interestingly, four of the 11 fairness libraries (i.e.,
Aequitas, Fairness Indicators, FairML, and Transparent AI) do not have any
mitigation approach implemented; they implemented only bias detection
approaches, or only contain bias datasets for experimentation.
\begin{table*}[t]
  %\def\arraystretch{1.5}
    \centering
    \caption{Bias mitigation approaches that are implemented as APIs in our selected API libraries}
    % \shaiful{My concern is we don't have a similar table for RQ2.}\ajoy{there are hundred of such metrics, so it not feasible to present them in a table. however, we mentioned some of the them as examples in the descriptions}
    \label{tab:mitigation_approach}
    \scalebox{0.8}{
    \begin{tabular}{llr}
    \toprule
    \textbf{Mitigation Approaches}  										&  \textbf{Introduced By}  &					 \textbf{Implemented in Fairness Libraries}  \\ \midrule
	\textit{Disparate impact remover}  & Feldman et al. (2015)  \cite{feldmanCertifyingRemovingDisparate2015}  & AI Fairness 360, BlackBoxAuditing, Fairness Comparison \\
    \textit{Learning fair representations} & Zemel et al. (2013)  \cite{zemelLearningFairRepresentations2013}	&	AI Fairness 360, EthicML \\
    \textit{Optimized preprocessing} & Calmon et al. (2017) \cite{calmonOptimizedPreProcessingDiscrimination2017}	& AI Fairness 360 \\
    \textit{Reweighing} & Kamiran et al. (2012) \cite{kamiranDataPreprocessingTechniques2012a} & AI Fairness 360, EthicML \\
    \textit{Massaging} & Kamiran et al. (2012) \cite{kamiranDataPreprocessingTechniques2012a} & EthicML \\
    Correlation remover	&	Fairlearn (Library) \cite{FairlearnDocumentationFairlearn} & Fairlearn \\
    \textit{Adversarially learned fair representations}	&	Beutel (2017) \cite{beutelDataDecisionsTheoretical2017}	&	EthicML	\\
    Upsampling	&	EthicML (Library) \cite{EthicMLDocumentationMitigation}	&	EthicML	\\
    \textit{Variational Fair Auto-Encoder}	&	Louizos et al. (2017) \cite{louizosVariationalFairAutoencoder2017}	&	EthicML	\\
    Relabelling	&	ThemisML (Library) \cite{bantilanThemisMLSource2017}	& ThemisML	\\
    \textit{Discrimination-Free Classification}	&	Calders et al. (2010) \cite{caldersThreeNaiveBayes2010}	&	Fairness Comparison \\
    \textit{Adversarial debiasing} & Zhang et al. (2018) \cite{zhangMitigatingUnwantedBiases2018}	&	AI Fairness 360	\\
    \textit{Gerry Fair classifier}	&	Kearns et al. (2018) \cite{kearnsPreventingFairnessGerrymandering2018}	&	AI Fairness 360, Gerryfair	\\
    \textit{Meta Fair classifier}	&	Celis et al. (2020) \cite{celisClassificationFairnessConstraints2020}	&	AI Fairness 360	\\
    \textit{Prejudice remover}	&	Kamishima et al. (2012)	\cite{kamishimaFairnessawareClassifierPrejudice2012}	&	AI Fairness 360, EthicML \\
    \textit{Exponentiated gradient reduction}	&	Agarwal et al. (2018) \cite{agarwalReductionsApproachFair2018}	&	AI Fairness 360, Fairlearn, EthicML \\
    \textit{Grid search reduction}	&	Agarwal et al. (2018) \cite{agarwalReductionsApproachFair2018}	&	AI Fairness 360, Fairlearn \\
	\textit{Distributionally-robust optimization}	&	Hashimoto et al. (2018) \cite{hashimotoFairnessDemographicsRepeated2018}	&	EthicML \\
    \textit{CORELS (Certifiably Optimal RulE ListS)}	&	Angelino et al. (2018) \cite{angelinoLearningCertifiablyOptimal2018}	&	EthicML \\
    \textit{Learning Classification without Disparate Mistreatment}	&	Zafar et al. (2017) \cite{zafarFairnessDisparateTreatment2017}	&	EthicML, Fairness Comparison \\
    \textit{Calibrated equalized odds}	&	Pleiss et al. (2017) \cite{pleissFairnessCalibration2017}	&	AI Fairness 360	\\
    \textit{Equalized odds} & Hardt et al. (2016) \cite{hardtEqualityOpportunitySupervised2016a} &	AI Fairness 360, Fairlearn, EthicML \\
    \textit{Reject option classification}	&	Kamiran et al. (2012) \cite{kamiranDecisionTheoryDiscriminationAware2012}	&	AI Fairness 360, ThemisML \\
    DP flip	&	EthicML (Library) \cite{FairlearnDocumentationFairlearn}	&	EthicML \\
    \bottomrule
\end{tabular}
}
\end{table*}


In order to have insights into how these mitigation approaches work, and how
they are used in the wild, we first merge these mitigation approaches into
higher-level more generic approaches. For example, we merge the
\textit{Correlation remover} and the \textit{Desperate impact remover}
mitigation APIs to higher-level \textit{data transformation}, because they
internally use different data transformation techniques to mitigate bias within
a dataset. These generic approaches were then merged into the three highest
level approaches, in accordance with previous
studies~\cite{mehrabiSurveyBiasFairness2021, bellamyAIFairness3602018a}, which
are known as pre-processing, in-processing, and post-processing.  The first two
authors went through the source materials of these mitigation approaches (e.g., original publications, tutorials, sample implementations) to
prepare this higher-level categorization. The authors first independently went through these source materials and then worked together until they reach an agreement about the categorization of these approaches. This process took $\sim$20 hours of online discussion.

% \rev{To note, it might happen that one repository uses several types of bias mitigation methods. To consider such cases, we consider each of those bias mitigation methods individually for counting the number of total methods used within those repositories. Similarly, if multiple approaches or algorithms are found within a single repository that repository was counted once individually for each of those mitigation approaches.}



%Figure~\ref{fig:mitigation_approach} summarizes the results, which we describe as follows.  
\subsubsection{Results}\label{sec:rq-bias-mitigation-results}
Figure~\ref{fig:mitigation_usecase_dist} shows that 68.2\% of the repositories that applied biased mitigation are within the Prediction activity type, followed by Operation and Analysis. 
% The top position of the Learning activity type is unsurprising because it is the most prevalent type in our dataset (Section~\ref{sec:lib_usecases}, Figure~\ref{fig:usecase_category}, and Section~\ref{sec:rq-bias-detection-strategies}, Table~\ref{tab:detection_usecases}).

Figure~\ref{fig:mitigation_domain_dist} shows the percentage distribution of the repositories that used these mitigation approaches across different use-case domains. 
% Consistent with our previous findings (e.g., Figure~\ref{fig:detection_domain_dist} in Section~\ref{sec:rq-bias-detection-strategies}), 
Here we see the Service domain as the most common domain; 59.1\% of all the repositories that use bias mitigation APIs are within this domain. The rest have been used within the Model domain (40.9\%).



\begin{figure}[t]
\subfloat[By activity types]
      {
      \centering\begin{tikzpicture}[scale=0.40]-
      \tikzstyle{every node}=[font=\footnotesize]
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=45,
         color={black!10, black!30, black!50, black!70},
        ]
        {
            % 64.2/\bf{Learning} (64.2\%),
            % 16/\bf{Analysis} (16\%),
            % 15/\bf{Prediction} (15\%),
            % 4.7/\bf{Operation} (4.7\%)
            %%%
            9/\bf{Analysis} (9\%),
            68.2/\bf{Prediction} (68.2\%),
            22.7/\bf{Operation} (22.7\%)
        }
    \end{tikzpicture}
    \label{fig:mitigation_usecase_dist}
      } 
\subfloat [By domains]
      {
      \centering\begin{tikzpicture}[scale=0.40]-
      \tikzstyle{every node}=[font=\footnotesize]
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=65,
         color={black!10, black!30, black!50, black!70, black!90},
        ]
        {
            % 79.2/\bf{Generic} (79.2\%),
            % 8.5/\bf{Model} (8.5\%),
            % 6.6/\bf{Legal} (6.6\%),
            % 3.8/\bf{Business} (3.8\%),
            % 1.9/\bf{Health} (1.9\%)
            %%%
            % 40.9/\bf{Model} (40.9\%),
            % 31.8/\bf{Legal} (31.8\%),
            % 18.2/\bf{Business} (18.2\%),
            % 9.1/\bf{Health} (9.1\%)
            %%%
            40.9/\bf{Model} (40.9\%),
            59.1/\bf{Service} (59.1\%)
        }
    \end{tikzpicture}
    \label{fig:mitigation_domain_dist}
      } 
      \caption{Distribution of use-cases of the repositories that used the bias mitigation approaches}
\vspace{-3mm}
\label{fig:mitigation_dist}    
\end{figure}
\begin{figure}[t]
\centering
%\includegraphics[width=0.8\columnwidth,keepaspectratio]{figs/analysis/mitigation_approaches.pdf}
\includegraphics[scale=0.6]{figs/analysis/mitigation_approaches.pdf}
\caption{Classification of bias mitigation approaches.}
\label{fig:mitigation_approach}
\end{figure}
%\nd\bf{\underline{Classification of mitigation approaches:}}


\fig\ref{fig:mitigation_approach} presents the distribution of overall used
mitigation approaches.
We see that In-processing is the most common approach to bias mitigation in our GitHub repositories (44.8\%), where the Fairness constraints (20.7\%) is the most dominant in-processing approach. Also, only 13.8\% of the projects followed the multi-objective optimization approach. 


% , which implies that most other projects did not directly worked on the drop in accuracy while minimizing bias. 
Along with that, we see the worst-case error minimization approach along with Neutralizing probability distribution were not adopted by any of our repositories. 

Next, we see 37.9\% of our GitHub projects adopted different pre-processing approaches for bias mitigation. Resampling is the most common pre-processing approach (20.7\% GitHub repositories), followed by Data transformation, the second most prevalent pre-processing approach (17.2\%). On the other hand, the learning fair representations approach~\cite{zemelLearningFairRepresentations2013}) has been applied by 6.9\% of the repositories. 

Finally, we find that 17.2\% of our subject repositories used post-processing
mitigation all of which came from the usage of the Probabilistic label change
approach, as the other post-processing approach, Random flipping, was not used by
any of the studied repositories.


% We see that Pre-processing is the most common approach to bias mitigation in our GitHub repositories (40.5\%). Data transformation is the most common pre-processing approach (21.2\% GitHub repositories), followed by Resampling, the second most prevalent pre-processing approach (19\%). On the other hand, the learning fair representations approach~\cite{zemelLearningFairRepresentations2013}) has been applied by 6\% of the repositories. 
% Next, we see 33.9\% of our GitHub projects adopted different in-processing approaches for bias mitigation. Fairness constraints (20\%) is the most dominant in-processing approach. Surprisingly, only 7.6\% of the projects followed the multi-objective optimization approach, which implies that most other projects did not directly worked on the drop in accuracy while minimizing bias. Along with that, we see the worst case error minimization approach was not adopted by any of our repositories. 
% Finally, we find that 25.6\% of our subject repositories used post-processing mitigation all of which came from the usage of the Probabilistic label change approach, as the other post-processing approach, Random flipping, was not used by any of the studied repositories.


% \begin{figure}
% \centering
% \subfloat
%       {
%       \centering\begin{tikzpicture}[scale=0.50]-
%       \tikzstyle{every node}=[font=\footnotesize]
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0, rotate=45,
%          color={black!10, black!30, black!50, black!70},
%         ]
%         {
%             40.5/\bf{Pre-processing} (40.5\%),
%             33.9/\bf{In-processing} (33.9\%),
%             25.6/\bf{Post-processing} (25.6\%)
%         }
%     \end{tikzpicture}
%       } 
% \caption{Distribution of the used bias mitigation approaches}
% \vspace{-3mm}
% \label{fig:mitigation_dist}    
% \end{figure}


% In  we present a classification of the bias mitigation approaches (mentioned in \tbl\ref{tab:mitigation_approach}).  
% \nd\bf{\underline{Mitigation Approaches based on Activity, Domains, and Use-cases:}}




Table~\ref{tab:mitigation_usecases} shows how different mitigation approaches
were used across different use-cases found in RQ1. Mitigation approaches are
indeed used across very different use-cases (i.e., different activities and
different domains) to reduce bias and improve the overall fairness of the
systems. We find that different repositories with the same
use case can apply different bias mitigation approaches. For example, the
repositories for credit approval (service domain in
Table~\ref{tab:mitigation_usecases}) have applied all three highest-level
mitigation approaches, and with different algorithms: pre-processing (with
resampling, and data transformation),  in-processing (with fairness constraints,
and regularization), and post-processing (with probabilistic label change). This
observation is also true for disease prediction within the service domain.


% \begin{table}[htbp]
%   %\def\arraystretch{1.5}
%     \centering
%     \caption{Usage of mitigation approaches in different use-cases \shaiful{it does not match with the previous figure where we found data transformation was the most prevalent pre-processing technique. You need to make everything consistent everywhere, otherwise we will get a direct rejection.}
%     \gias{for the column use case, show a bar chart of the distribution of use case domains per use case category. to produce the bar chart see Table VII from \url{https://arxiv.org/pdf/2201.04241.pdf}}}
%     \label{tab:mitigation_usecases}
%     \scalebox{0.8}{
%     \begin{tabular}{llllr}
%     \toprule
%     \textbf{Mitigation}  	&  \textbf{Mitigation}  &		 \textbf{Use-case}  &			 \textbf{Use-cases}  &  \textbf{Repository}\\
%     \textbf{Category}  	&  \textbf{Sub-Category}  &		 \textbf{Category}  &			 						&	 \textbf{Count} \\ \midrule
% Pre-processing & Resampling & Learning & Generic (Mitigation, Detection, API Usage) & 36 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring) & 11 \\
%  &  & Prediction & Business (Credit Approval, Advertisement Strategy), Health (Disease Prediction), \\
%  &  &   &   Model (Recommendation), Legal (Risk Detection, Action Prediction) & 10 \\
%  &  & Operation & Model (Development) & 1 \\
% \cline {2-5}
%  & Data transformation & Learning & Generic (Mitigation, Detection, API Usage) & 25 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring), Model (Monitoring) & 11 \\
%  &  & Prediction & Business (Credit Approval) & 3 \\
%  &  & Operation & Model (Development) & 1 \\
% \cline {2-5}
%  & Relabelling & Learning & Generic (Mitigation) & 1 \\
% \cline {2-5}
% \cline {1-5}
% In-processing & Fairness constraints & Learning & Generic (Mitigation, Detection, API Usage) & 33 \\
%  &  & Prediction & Generic (Survivability Prediction), Health (Disease Prediction),  \\
%  &  &   &  Business (Credit Approval), Legal (Risk Detection, Legal Status Prediction) & 7 \\
%  &  & Operation & Model (Development) & 4 \\
%  &  & Analysis & Model (Model Security), Generic (Fairness Impact, Monitoring) & 3 \\
% \cline {2-5}
%  & Multi objective & Learning & Generic (Mitigation, API Usage) & 13 \\
%  & ~optimization & Prediction & Health (Disease Prediction), Business (Credit Approval), Legal (Risk Detection) & 5 \\
%  &  & Analysis & Generic (Fairness Impact, Monitoring), Model (Monitoring) & 4 \\
%  &  & Operation & Model (Development) & 2 \\
% \cline {2-5}
%  & Regularization & Learning & Generic (Mitigation, API Usage) & 11 \\
%  &  & Prediction & Business (Credit Approval), Legal (Risk Detection, Action Prediction) & 5 \\
%  &  & Analysis & Generic (Monitoring) & 3 \\
%  &  & Operation & Model (Development) & 1 \\
% \cline {2-5}
% \cline {1-5}
% Post-processing & Probabilistic & Learning & Generic (Mitigation, Detection, API Usage) & 32 \\
%  &  ~label change & Prediction & Health (Disease Prediction), Model (Language Analysis),  \\
%  &  &   &  Business (Credit Approval), Legal (Risk Detection) & 6 \\
%  &  & Analysis & Model (Model Security), Generic (Fairness Impact, Monitoring) & 6 \\
%  &  & Operation & Model (Development) & 1 \\
% \cline {2-5}
% \cline {1-5}
% \end{tabular}
% }
% \end{table}

% \begin{table}[t]
%   %\def\arraystretch{1.5}
%     \centering
%     \caption{Usage of mitigation approaches in different use-cases. Here each color bar denotes a domain type 
%     (Black = Generic, Green = Model, Red = Business, Blue = Legal, Orange = Health). \#R = Number of GitHub repositories}
%     \label{tab:mitigation_usecases}
%     %\scalebox{0.8}{
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lll|l}
%     \toprule
%     \textbf{Mitigation}  &	\textbf{Use-case Activity}  &  \textbf{\#R} & \textbf{\% Repos With of Use-case Domain} \\ \toprule
%     %\textbf{Category}  	&  \textbf{Sub-Category}  &		 \textbf{Category}      &	\textbf{Count} & \textbf{Domains} \\ \midrule
% \bf{Pre-processing} & Learning & 36 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Resampling  & Analysis & 11 & \sixbars{100}{0}{0}{0}{0}{0} \\
%  & Prediction & 10 & \sixbars{0}{9}{0}{27}{45}{18} \\
%  & Operation & 1 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% & Learning & 25 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Data transformation  & Analysis & 11 & \sixbars{87}{13}{0}{0}{0}{0} \\
%   & Prediction & 3 & \sixbars{0}{0}{0}{100}{0}{0} \\
%   & Operation & 1 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% Relabelling & Learning & 1 & \sixbars{100}{0}{0}{0}{0}{0} \\
% %\cmidrule {2-4}
% \midrule
% \bf{In-processing} & Learning & 33 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Fairness constraints  & Prediction & 7 & \sixbars{14}{0}{0}{29}{29}{29} \\
%  & Operation & 4 & \sixbars{0}{100}{0}{0}{0}{0} \\
%  & Analysis & 3 & \sixbars{75}{25}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% Multi objective optimization & Learning & 13 & \sixbars{100}{0}{0}{0}{0}{0} \\
%  & Prediction & 5 & \sixbars{0}{0}{0}{40}{40}{20} \\
%  & Analysis & 4 & \sixbars{75}{25}{0}{0}{0}{0} \\
%  & Operation & 2 & \sixbars{0}{100}{0}{0}{0}{0} \\
% \cmidrule {2-4}
% Regularization & Learning & 11 & \sixbars{100}{0}{0}{0}{0}{0} \\
%  & Prediction & 5 & \sixbars{0}{0}{0}{40}{60}{0} \\
%   & Analysis & 3 & \sixbars{100}{0}{0}{0}{0}{0} \\
%  & Operation & 1 & \sixbars{0}{100}{0}{0}{0}{0} \\
% %\cmidrule {2-4}
% \midrule
% \bf{Post-processing} & Learning & 32 & \sixbars{100}{0}{0}{0}{0}{0} \\
% Probabilistic label change  & Prediction & 6 & \sixbars{0}{17}{0}{33}{33}{17} \\
%   & Analysis & 6 & \sixbars{91}{9}{0}{0}{0}{0} \\
%  & Operation & 1 & \sixbars{0}{100}{0}{0}{0}{0} \\
% %\cline {2-5}
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
  %\def\arraystretch{1.5}
    \centering
    \caption{Usage of mitigation approaches in different use-cases. Here each color bar denotes a domain type 
    (Black = Model and Green = Service). \#R = Number of GitHub repositories}
    \label{tab:mitigation_usecases}
    %\scalebox{0.8}{
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lll|l}
    \toprule
    \textbf{Mitigation}  &	\textbf{Non-generic Use-case}  &  \textbf{\#R} & \textbf{\% Repos With of Use-case Domain} \\ \toprule
\bf{Pre-processing }  &  &  &  \\
\textit{Resampling}  & Prediction & 10 & \sixbars{9}{91} \\
Non-generic: 11
%Generic: 47  
& Operation & 1 & \sixbars{100}{0} \\
% & & & \\
\cmidrule {2-4}
\textit{Data transformation} & Prediction & 3 & \sixbars{0}{100} \\
Non-generic: 5 
%Generic: 35  
& Analysis & 1 & \sixbars{100}{0} \\
  & Operation & 1 & \sixbars{100}{0} \\
%\cmidrule {2-4}
%\textit{Relabelling} & \multicolumn{3}{c}{Generic: 1} \\
%\cmidrule {2-4}
\midrule
\bf{In-processing}  &  &  &  \\
\textit{Fairness constraints}  & Prediction & 6 & \sixbars{0}{100} \\
Non-generic: 11 
%Generic: 36 
& Operation & 4 & \sixbars{100}{0} \\
 & Analysis & 1 & \sixbars{100}{0} \\
\cmidrule {2-4}
\textit{Multi-objective optimization} & Prediction & 5 & \sixbars{0}{100} \\
Non-generic: 8
%Generic: 16 
& Operation & 2 & \sixbars{100}{0} \\
  & Analysis & 1 & \sixbars{100}{0} \\
\cmidrule {2-4}
\textit{Regularization} & Prediction & 5 & \sixbars{0}{100} \\
Non-generic: 6  
% Generic: 14  
& Operation & 1 & \sixbars{100}{0} \\
%& & & \\
%\cmidrule {2-4}
\midrule
\bf{Post-processing}  &  &  &  \\
\textit{Probabilistic label change} &  Prediction & 6 & \sixbars{17}{83} \\
Non-generic: 8 
% Generic: 37   
& Analysis & 1 & \sixbars{100}{0} \\
 & Operation & 1 & \sixbars{100}{0} \\
%\cline {2-5}
\bottomrule
\end{tabular}%
}
\end{table}



% However, mitigation and API usage across various domains. 

In Listing \ref{lst:usecase1_mitigation}, we show how bias was mitigated, using
the \textit{Reweighing} pre-processing algorithm
\cite{kamiranDataPreprocessingTechniques2012a}, in the metropolitan police use
case described in \sec\ref{sec:rq-bias-detection-strategies}.
After applying the mitigation algorithm the repository developers generally
verify whether the situation improved or not by re-calculating bias detection
metrics. For example, here \textit{BinaryLabelDatasetMetric} has been used for
recalculating the dataset metric.
%\shaiful{In the detection section, you have an example for hospitalization. If you can not show the mitigation for hospitalization, then replace the hospitalization example with something else (something interesting) in both places. But when you do, check for consistency everywhere. Also, don't break the style.}

\begin{lstlisting}[caption={Use-case1: Mitigating bias and recalculating bias metrics},label={lst:usecase1_mitigation},basicstyle=\footnotesize]
rw =  <@\textcolor{black}{\colorbox{yellow}{Reweighing}}@>(unprivileged_groups=unprivileged_groups,
                privileged_groups=privileged_groups)
train_pp_bld_f = rw.fit_transform(train_pp_bld)

metric_train_bld = <@\textcolor{black}{\colorbox{yellow}{BinaryLabelDatasetMetric}}@>(train_pp_bld_f,
                  unprivileged_groups=unprivileged_groups,
                    privileged_groups=privileged_groups)
\end{lstlisting}

% This use-case example (denoted as Use-case4) is a research-oriented project from \href{https://github.com/spring-epfl/disparate-vulnerability}{spring-epfl/disparate-vulnerability} repository that focused on analyzing Membership Inference attack against an ML model. 

% \begin{lstlisting}[caption={Use-case4: Using bias mitigation approaches},label={lst:usecase4_mitigation},basicstyle=\footnotesize]
% from fairlearn.reductions import (
%     GridSearch,
%     ExponentiatedGradient,
%     ErrorRateParity,
%     DemographicParity,
%     EqualizedOdds,
% )

% from fairlearn.postprocessing import (
%     ThresholdOptimizer
% )
% \end{lstlisting}





% % Usecase 5: https://github.com/julian-zucker/arbiter 
% \begin{lstlisting}[caption={Use-case5: Imports},label={lst:usecase5_imports},basicstyle=\footnotesize]
% from aif360.datasets import BinaryLabelDataset
% from aif360.algorithms.inprocessing import AdversarialDebiasing
% from sklearn.ensemble import RandomForestClassifier
% from aif360.metrics import ClassificationMetric


% dataset = BinaryLabelDataset(
%     df=DataFrame(data),
%     protected_attribute_names={protected_attribute_name},
%     label_names={label_name},
%     favorable_label=2,
%     unfavorable_label=1,
% )
% \end{lstlisting}


% \begin{lstlisting}[caption={Use-case5: Mitigating bias},label={lst:usecase5_mitigation},basicstyle=\footnotesize]
% debiaser = <@\textcolor{black}{\colorbox{yellow}{AdversarialDebiasing}}@>(
%     unprivileged_groups=({protected_attribute_name: 0},),
%     privileged_groups=({protected_attribute_name: 1},),
%     scope_name="debiaser",
%     debias=True,
%     sess=sess,
% )
% debiaser.fit(train)

% model = RandomForestClassifier(class_weight="balanced")
% X_tr = np.delete(train.features, protected_attribute_index, axis=1)
% y_tr = train.labels.ravel()
% model.fit(X_tr, y_tr)

% test_pred = test.copy(deepcopy=True)
% test_pred.scores = model.predict(np.delete(debiaser.predict(test).features, protected_attribute_index, axis=1))

% accuracy = np.sum(np.equal(test.scores, test_pred.scores))
% \end{lstlisting}


% \begin{lstlisting}[caption={Use-case5: Validating after mitigating bias},label={lst:usecase5_validation},basicstyle=\footnotesize]
% disparate_impact = <@\textcolor{black}{\colorbox{yellow}{ClassificationMetric}}@>(
%     test,
%     test_pred,
%     unprivileged_groups=({protected_attribute_name: 0},),
%     privileged_groups=({protected_attribute_name: 1},),
% ).<@\textcolor{black}{\colorbox{yellow}{disparate\_impact}}@>()

% print(f"Accuracy: {accuracy}")
% print(f"Disparate impact: {disparate_impact}")
% if disparate_impact > float(required_fairness):
%     raise ValueError(
%         f"Too unfair! Disparate impact was {disparate_impact} but must be less than {required_fairness}"
%     )
% \end{lstlisting}



% % Usecase 6: https://github.com/RossyNguyen/BIT---Healthcare-Bias-Dection-tool 
% \begin{lstlisting}[caption={Use-case6: Imports},label={lst:usecase6_imports},basicstyle=\footnotesize]
% from aif360.datasets import BinaryLabelDataset
% from aif360.metrics import BinaryLabelDatasetMetric, ClassificationMetric
% from aif360.algorithms.preprocessing import Reweighing

% protected_attribute = 'ethnicity'
% dataset = load_preproc_data_heart([protected_attribute])

% privileged_groups = [{protected_attribute:1}]
% unprivileged_groups = [{protected_attribute:2}, {protected_attribute:3}, {protected_attribute:4}, {protected_attribute:5},{protected_attribute:6}]
% \end{lstlisting}


% \begin{lstlisting}[caption={Use-case6: Mitigating bias},label={lst:usecase6_mitigation},basicstyle=\footnotesize]
% metric_orig_train = BinaryLabelDatasetMetric(data_orig_train,
%                                             unprivileged_groups=unprivileged_groups,
%                                             privileged_groups=privileged_groups
%                                                 )
% print("Mean {}".format(metric_orig_train.mean_difference()))

% rw = Reweighing(unprivileged_groups = unprivileged_groups, privileged_groups=privileged_groups)
% data_transf_train = rw.fit_transform(data_orig_train)
% metric_transf_train = BinaryLabelDatasetMetric(data_transf_train, unprivileged_groups=unprivileged_groups, privileged_groups = privileged_groups)

% print("Mean difference after transformation =%f " % metric_transf_train.mean_difference())
% \end{lstlisting}


% \begin{lstlisting}[caption={Use-case6: Validating after mitigating bias},label={lst:usecase6_validation},basicstyle=\footnotesize]
% def calculate_bias_measures(data_orig_train, data_orig_vt, unprivileged_groups, privileged_groups):
%     model = RandomForestClassifier().fit(data_orig_train.features, data_orig_train.labels.ravel(), sample_weight=data_orig_train.instance_weights)
%     dataset = data_orig_vt
%     dataset_pred = dataset.copy()
%     dataset_pred.labels = model.predict(data_orig_vt.features)
%     classified_metric_race = ClassificationMetric(dataset, dataset_pred,
%                                                   unprivileged_groups=unprivileged_groups,
%                                                   privileged_groups=privileged_groups
%                                                   )
%     metric_pred_race = BinaryLabelDatasetMetric(dataset_pred,
%                                                 unprivileged_groups=unprivileged_groups,
%                                                   privileged_groups=privileged_groups
%                                                  )
%     print("Mean difference {}".format(metric_pred_race.mean_difference()))
%     print("Disparate Metric {}".format(metric_pred_race.disparate_impact()))
%     print("Equal Opportunity Difference {}".format(classified_metric_race.equal_opportunity_difference()))
%     print("Average Abs Odds Difference {}".format(classified_metric_race.average_abs_odds_difference()))
%     print("Theil index {}".format(classified_metric_race.theil_index()))

% ............

% calculate_bias_measures(data_orig_train, data_orig_vt, unprivileged_groups, privileged_groups)
% calculate_bias_measures(data_orig_valid, data_orig_test, unprivileged_groups, privileged_groups)
% \end{lstlisting}



\begin{figure}[t]
\centering
\subfloat[Evolution of different types of mitigation approaches at the highest level.]
      {
      \centering
      \includegraphics[scale=.55]{figs/analysis/mitigation-type-trends-filtered.pdf}
      \label{fig:mitigation-type-trends}
      } \\
\subfloat [Evolution of different types of mitigation algorithms.]
      {
      \centering
      \includegraphics[scale=.55]{figs/analysis/mitigation-subtype-trends-filtered.pdf}
      \label{fig:mitigation-subtype-trends}
      } 
      \caption{Evolution of bias mitigation approaches based on the integration of the APIs on corresponding GitHub repositories.}
\vspace{-3mm}
\label{fig:mitigation-trends}    
\end{figure}



\fig\ref{fig:mitigation-trends} shows how the use of different types of bias
mitigation approaches evolved over the years. 
To perform this trend analysis, we used a similar approach that we followed for analyzing the trends of usage of the detection APIs (described in \sec\ref{sec:rq-bias-detection-results}). 
\fig\ref{fig:mitigation-type-trends} shows the trend at the highest level (i.e.,
Pre-processing, In-processing, and Post-processing). Pre-processing---removing
bias from training data---has always been the most dominant mitigation approach.
In-Processing, although less popular at the beginning, has become the most
popular approach over time. On the other hand, even though Post-processing has been the
least popular of the three, one of its algorithms, probabilistic label change, has always been
the most dominant bias mitigation approach until 2021
(Figure~\ref{fig:mitigation-subtype-trends}) when steadily rising fairness constraints approach took over its place.
In general, we observe an overall increase in using bias mitigation in ML
software. This implies the growing demand for fairness improvement and bias mitigation in ML systems.


\begin{rqbox}{RQ3 Summary} 
% There are 23 different bias mitigation approaches (in three highest-level categories) implemented as APIs in the 11 selected libraries. However, only 15 of these mitigation approaches were found in our studied GitHub repositories. Bias mitigation is applied in repositories with very different use-cases and domains. 
% Demand for bias mitigation in machine learning software is increasing over time.
% Pre-processing to remove bias from the training data is the most prevalent bias
% mitigation approach. However, the other two approaches---in-processing, and
% post-processing---are also common. We observe that, in many use-cases, bias can
% be removed with multiple approaches; therefore, a comparison of their performance
% could be useful. 
The primary implications of our observations are two.  i) Demand for bias mitigation in machine learning software is increasing over time. This is an important observation for the research community who, therefore, should focus on building more bias mitigation approaches and should investigate more on solving the current mitigation-related problems, such as making a bias mitigation approach to be transferable~\cite{jin2020transferability}. ii) Although the in-processing approaches are the most common bias mitigation approach, for the same use cases bias can be mitigated by multiple approaches. As such, there is a need to study which mitigation approach is better in a given scenario, which may act as a guideline for the developers. 

\end{rqbox}

\subsection{RQ4. What are the topics found in the issues that developers reported while using the API libraries?}\label{sec:challenges-bias-apis}
\subsubsection{Motivation} Our findings in RQ1 - RQ3 show that the fairness API libraries are used to support diverse use case scenarios to detect and mitigate biases. 
We also find that a considerable number of the applications focus on tutorials or generic usage, which could denote that the users of the API libraries need to spend time and effort 
learning how to use the API libraries before they apply those to real-world use cases (e.g., healthcare). As such, it is important to understand whether the API libraries can be improved and/or 
adapted to support and increase their usage. To understand how the API libraries can be improved, we first need to understand the types of challenges the developers and users of the API libraries face while using and developing the API libraries. This insight can help the developers of the API libraries to better design their API libraries along with the key topic areas of challenges.
\subsubsection{Approach} To understand the challenges the API developers of fairness libraries
face, we applied topic modeling on the 2581 GitHub issue discussions (613 issue reports and 1968 associated
comments) of these libraries that we collected in \sec\ref{sec:collect-issue-comments}. 

% \rev{ Instead of combining the issue reports and the associated issue comments together, we considered these two types of texts separately within our dataset. If we force all comments and issue descriptions of a given issue into a single document sample, the topic modeling of that document might produce extremely noisy output as that combined document might contain discussions on several topics. In fact, the authors initially considered all comments under a discussion as one single entity, but then found out that the comments from a discussion can be categorized under different areas. For example, issues such as \href{https://github.com/fairlearn/fairlearn/issues/265}{fairlearn/issues/265} and \href{https://github.com/Trusted-AI/AIF360/issues/51}{AIF360/issues/51} contains discussion of topics ranging from bias APIs specific issues to troubleshooting, installation problem, etc. which would produce noisy topic if all of their discussions are considered within a single entity. On the other hand, just because each comment has been considered as a separate entity,  it does not necessarily mean they would produce different topics. Multiple comments from a discussion can be under a single topic if they have similar discussions.}
\rev{
Instead of combining the issue reports and the associated issue comments together, we considered these two types of texts separately. Initially, we merged all comments and issue descriptions of a given issue into a single document sample. The results after topic modeling become extremely noisy with this approach. This is because developers often discuss issues containing multiple topics. For example, the issue \href{https://github.com/fairlearn/fairlearn/issues/265}{fairlearn/issues/265} and \href{https://github.com/Trusted-AI/AIF360/issues/51}{AIF360/issues/51} contain discussions ranging from bias APIs specific issues to troubleshooting, installation problem, etc. This would produce noisy topics if all of their discussions are considered within a single entity. On the other hand, just because each comment has been considered as a separate entity, it does not necessarily mean they would produce different topics. Multiple comments from a discussion can be under a single topic if they have similar discussions.
}

Our approach to topic modeling is similar to~\cite{scocciaChallengesDevelopingDesktop2021}, where
Scoccia \textit{et al.} analyzed the challenges in developing desktop web apps
using the issue reports from the apps' repositories that are hosted on GitHub. We apply topic modeling and analyze the output of topic modeling as follows.

First, we preprocess the issue discussions. We consider the issue titles,
the issue bodies, and the comment bodies as text fields. We then applied 
noise-reducing steps following previous
studies~\cite{uddinEmpiricalStudyIoT2021,alaminEmpiricalStudyDeveloper2021}. We
first removed all the code segments and HTML tags used to mark non-text blocks.
Then we removed stop words (i.e., ``a'', ``the'', ``this'', etc.), numbers,
non-alphabetical characters, and punctuation marks. We then applied Porter
stemming to get the roots of the words. After this step, we were left with 2540 issue discussions due to the removal of noisy and empty discussions.

Second, we apply topic modeling to the preprocessed issue contents. Similar to
the existing studies
(e.g.,~\cite{uddinEmpiricalStudyIoT2021,alaminEmpiricalStudyDeveloper2021}), we
used the \emph{Latent Dirichlet Allocation} (LDA) algorithm
\cite{bleiLatentDirichletAllocation} provided by the MALLET library
\cite{mccallumMALLETMachineLearning}. The algorithm provides a list of topics to
group the issue discussion texts into \textit{T} topics, taking the
pre-processed texts as input. To find the optimal number of topics, we followed
the standard practice proposed by Arun \textit{et
al.}~\cite{arunFindingNaturalNumber2010}.  We have utilized the c.v. metric from
the \texttt{GenSim} package~\cite{rehurekSoftwareFrameworkTopic2010} for
calculating the coherency scores for each of these topics, and used this score
to get the optimal number of topics, as done by previous studies~
\cite{uddinAutomaticSummarizationAPI2017,uddinEmpiricalStudyIoT2021,alaminEmpiricalStudyDeveloper2021}.
As the two hyper-parameters of LDA, we used $\alpha = 50/T$ and $\beta = 0.01$
and applied MALLET LDA for $T = {5~to~50}$, incremented by 1. The highest
coherency score generated by LDA was 0.54 for $T=10$ and for $T = 20$ topics.
However, after the first two authors went through several $T < 30$ topics (e.g.,
10 and 20 topics), they found that the generated topics were quite noisy and
contained multiple types of discussions in one single topic. So the authors took
the highest coherency score where $T > 30$, and found that $T=33$ topics---with
a coherence score of 0.53, pretty close to the highest score of 0.54---leads
less noisy topics. Subsequently, 33 was selected as the optimal
number of topics. 
% that should show 33 types of challenges developers face while
% developing and using fairness libraries.

Third, we manually label each topic. The label of a topic summarizes the
underlying concepts of that topic. For labeling the topics, we applied an open
card sorting approach \cite{williamCardSorting2013}, which is popular in the
community for labeling LDA-generated
topics~\cite{bagherzadehGoingBigLargescale2019,uddinEmpiricalStudyIoT2021}. In
this approach, a list of top words (10 words in our case) within a topic is used
along with a list of randomly selected text samples (10 samples in our case) to
find the label of a topic. Two of the authors labeled these topics by
synchronously communicating together using Skype and Zoom meetings. They only
labeled the topics after reaching a complete agreement over the labels; in case
of a few disagreements, the third author was involved. After the first round of
labeling, we merged a number of similar topics together as they indicate
identical issues. For example, topics 21 and 4 were merged into the same topic,
\emph{Installation}, as both of these topics discussed different
installation-related challenges. At the end of the discussion and merging
similar topics, we obtained 19 unique topics, which shows the 19 unique
challenges the developers face while developing or deploying fairness libraries.

Fourth, we build a hierarchy of the found topics. Given the fairness API libraries are used to improve the detection and mitigation of bias in 
ML software systems during the design and development of such software, we followed Alamin and Uddin~\cite{alalaminQualityAssuranceChallenges2021} and used the stages
of SDLC (Software Development Life Cycle) to build our higher-level topic category. For example,
\emph{Troubleshooting}, \emph{Testing}, and \textit{Fixing Warning} all are
related to maintaining the implementation of the API library, so we grouped
these together under the ``Maintenance'' category. This whole process took $\sim$25 hours of discussion.

\begin{figure}[t]
\centering
\includegraphics[scale=.55]{figs/analysis/topic_percentage_horizontal_80.pdf}
\caption{Distribution of topics by the total number of issue discussions.}
\label{fig:topic_percentage}
\end{figure}
\subsubsection{Results}
\fig\ref{fig:topic_percentage} shows the distribution of the 19 unique topics in our dataset of 2581 issue discussions. 
The topics are ordered based on the total number of issue discussions assigned to each topic. 
For example, the topic containing general opinions and reviews about the API libraries has the most number of issue discussions (14.6\% of all issue discussions), followed 
by discussions related to troubleshooting of the APIs (11.8\% of issue discussions) and the design and adoption of the bias mitigation methodologies in the APIs (11.2\% of issue discussions). 
On the contrary, the least number of discussions in the issue discussions happened around topics like model development (0.9\% of issue discussions) and the analysis of fixing warnings (0.4\% of issue discussions).

Figure~\ref{fig:topic_classify} shows the taxonomy of the topics created by organizing the 19 topics into a hierarchy. As our categorization is based on the stages of SDLC, we have
six categories describing the different stages of the SDLC: Requirement analysis,
Design, Development, Deployment, Validation, and Maintenance. We describe these
categories in detail as follows.
% Issues that are directly connected to ML/Fairness have the highest percentage (60.3\% of discussions, 12 topics), followed by Deployment (19\% of discussions, 3 topics), Bug (14\% of discussions, 3 topics), and UI (6.7\% of discussions, 1 topic). 

% \begin{figure}
% \centering
% \subfloat
%       {
%       \centering\begin{tikzpicture}[scale=0.40]-
%       \tikzstyle{every node}=[font=\footnotesize]
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0, rotate=170,
%          color={black!10, black!30, black!50, black!70},
%         ]
%         {
%             60.3/\bf{ML/Fairness}\\(60.3\% of Discussions\\ 12 Topics),
%             14/\bf{Bug}\\(14\% of Discussions\\ 3 Topics),
%             19/\bf{Deployment}\\(19\% of Discussions\\ 3 Topics),
%             6.7/\bf{UI}\\(6.7\% of Discussions\\ 1 Topic)
%         }
%     \end{tikzpicture}
%       } 
% \caption{Distribution of the issue discussions and topics per topic category}
% \vspace{-3mm}
% \label{fig:topic_dist}    
% \end{figure}

% \fig\ref{fig:topic_classify} presents the classification of the topics grouped into categories and subcategories. The percentage presented with each category and topic label represents the percentage of discussion comments within its parent category. For example, within the Methodology subcategory Bias Mitigation Methodologies had been discussed in 89.9\% of issues discussions and Feature Engineering methodology had been discussed in 11.1\% of the discussions. 


\begin{figure}[t]
\centering
\includegraphics[scale=.5]{figs/analysis/topic_categ_sunburst_edited.pdf}
\caption{Issue discussion topics with categories and subcategories}
\label{fig:topic_classify}
\end{figure}

% \fig\ref{fig:topic_percentage} shows the ordered list of found topics sorted by the number of discussion posts each of the topics dominates. 

\nd\bf{(1) Requirement Analysis Related Topics.} This category has the highest coverage (31.3\% of discussions, 5 topics), which contains discussions related to analyzing the requirements of developing fair ML models. More specifically, it contains discussions or queries regarding how to use the bias detection and mitigation approaches correctly and efficiently. The five topics within this category are:   
\begin{enumerate}[(i)]
\item Opinion, which contains queries related to asking opinions about fairness API-related problems. For example, it contains issues about if API developers should change the development process (e.g., \href{https://github.com/fairlearn/fairlearn/issues/853}{fairlearn/issues/853}), use certain external package as dependency or implement it (e.g., \href{https://github.com/fairlearn/fairlearn/issues/431#issuecomment-632558930}{fairlearn/issues/431\#issuecomment-632558930}).
\item Research, which contains discussion regarding researching around certain fairness topics. For example, going over research papers to improve the design of the fairness APIs (e.g., \href{https://github.com/fairlearn/fairlearn/issues/413#issuecomment-646236707}{fairlearn/issues/413\#issuecomment-646236707}).
\item Dataset usage, which contains queries about the usage of datasets supported by the API libraries. For example, what to do about certain dataset which throws error (e.g., \href{https://github.com/fairlearn/fairlearn/issues/95#issuecomment-561857634}{fairlearn/issues/95\#issuecomment-561857634}).
\item Understanding fairness definition contains queries to understand the definition of fairness in certain contexts or to report issues regarding invalid or inconsistent use of fairness definitions. For example, suggesting to reconsider the use of the words \emph{bias} and \emph{prejudice}, in a library's README file (e.g., \href{https://github.com/Trusted-AI/AIF360/issues/97}{AIF360/issues/97}).
\item User Interface (UI), which primarily contains discussions about UI components that can be found in these libraries. These UI components generally help in supporting the visualization of various outputs and metrics. For example, the discussion about a UI widget not working properly is part of this topic (e.g., \href{https://github.com/tensorflow/fairness-indicators/issues/143#issuecomment-696298372}{fairness-indicators/issues/143\#issuecomment-696298372}). 
\end{enumerate}


\nd\bf{(2) Design Related Topics.} This category contains discussions or queries about the methodology of designing certain features utilizing the support provided by the API libraries. This category consists of two topics:
\begin{inparaenum}[(i)]
\item Bias mitigation, which contains queries regarding the use of bias mitigation methods. For example, asking for suggestion on how to use certain bias mitigation approach (e.g., \href{https://github.com/fairlearn/fairlearn/issues/23#issuecomment-531314496}{fairlearn/issues/23\#issuecomment-531314496}).
\item Feature engineering, which contains queries related to applying feature engineering techniques or selecting features. For example, querying about how to use multiple sensitive features together (e.g., \href{https://github.com/fairlearn/fairlearn/issues/376}{fairlearn/issues/376}).
\end{inparaenum}


\nd\bf{(3) Development Related Topics.} Development consists of discussion around developing ML model or implementing fairness APIs. This category contains three topics: 
\begin{inparaenum}[(i)]
\item Model development contains discussion related to developing and hyper-parameter tuning of developed ML model. For example, this topic contains discussion on generalizing ML model (e.g., \href{https://github.com/fairlearn/fairlearn/issues/460}{fairlearn/issues/460}), and discussion on overfitting issue of the ML model (e.g., \href{https://github.com/fairlearn/fairlearn/issues/460#issuecomment-644245257}{fairlearn/issues/460\#issuecomment-644245257}).
\item Documentation contains queries related to API documentation of the libraries. For example, asking for updating certain image in the documentation (e.g., \href{https://github.com/fairlearn/fairlearn/issues/463}{fairlearn/issues/463}), and query regarding how to build the documentation (e.g., \href{https://github.com/fairlearn/fairlearn/issues/886#issuecomment-877001388}{fairlearn/issues/886\#issuecomment-877001388}). 
\item API expansion contains discussion around feature requests to expand the list of the supported APIs. For example, asking to add new fairness aware algorithm as a new API  (e.g., \href{https://github.com/fairlearn/fairlearn/issues/956}{fairlearn/issues/956}), and asking to implement new sets of fairness metrics  (e.g., \href{https://github.com/dssg/aequitas/issues/48}{aequitas/issues/48}) are under this topic.
\end{inparaenum}

\nd\bf{(4) Deployment Related Topics.} This category focuses on deployment-related issues that the developers and the users generally face, and consists of three related topics.
\begin{inparaenum}[(i)]
\item Artifact generation and bench-marking, which contains discussions related to artifact generation  such as package, dashboard  (e.g., \href{https://github.com/fairlearn/fairlearn/issues/322}{fairlearn/issues/322}), documentation, and benchmarking the tests (e.g., \href{https://github.com/fairlearn/fairlearn/issues/278}{fairlearn/issues/278}).
\item Dependency and Release contains problems related to library dependency and release of API libraries. For example,  the discussion on an issue related to multiple sets of dependency versions for a certain dependency (\href{https://github.com/fairlearn/fairlearn/issues/915#issuecomment-894399838}{fairlearn/issues/915\#issuecomment-894399838}) is within this topic. 
\item Installation and shell commands contain discussions related to the installation of the libraries or their dependencies and shell commands that can be used as alternative means to access the API features as a command-line utility. For example, this topic contains a discussion about installation issues on certain operating systems (\href{https://github.com/Trusted-AI/AIF360/issues/44}{AIF360/issues/44}).
\end{inparaenum}






\nd\bf{(5) Validation Related Topics.}  This category contains discussion related to validation of the developed fair ML model. The three categories that fall under this topic are:
\begin{inparaenum}[(i)]
\item Bias detection metrics validation, which contains query regarding how to validate which bias detection metrics to apply in a certain scenario. For example, the question about how to differentiate between two bias detection metrics (\href{https://github.com/fairlearn/fairlearn/issues/466#issuecomment-649096969}{fairlearn/issues/466\#issuecomment-649096969}) is within this topic.
\item Metrics operation contains queries related to metrics operations or requests to add new metrics. For example, the request to add new bias detection metrics (\href{https://github.com/fairlearn/fairlearn/issues/804}{fairlearn/issues/804}) is within this category. 
\item Performance measurement contains issues related to performance. For example, this topic contains the issue about the limitation of an existing performance measurement API (\href{https://github.com/fairlearn/fairlearn/issues/756}{fairlearn/issues/756}).
\end{inparaenum}

\nd\bf{(6) Maintenance Related Topics.} This is the third-largest category (14\% of the discussions) and consists of three topics that primarily focus on maintaining the source code of the API libraries. The three topics that are under this category are:
\begin{inparaenum}[(i)]
\item Troubleshooting, which contains bug reporting and bug fixing discussions. 
For example, reporting storage-related bugs while using an API (\href{https://github.com/fairlearn/fairlearn/issues/322}{fairlearn/issues/322}).
\item Testing contains discussions regarding test failure or test adequacy of the libraries. For example, discussion about test failure issues for some supplied examples (\href{https://github.com/fairlearn/fairlearn/issues/265}{fairlearn/issues/265}).
\item Fix warnings topic contains discussion on fixing warnings that can be generated in various phases of 
using the API library or the documentation. For example, a request to fix warnings in the documentation building phase (\href{https://github.com/fairlearn/fairlearn/issues/852}{fairlearn/issues/852}) is under this topic.
\end{inparaenum}



% Out of 19 topics, queries asking for an opinion on certain areas are found in the greatest number of issue discussions (14.6\%), followed by Troubleshooting which contains queries reporting and solving troubleshooting problems (11.8\%). 
% Figure~\ref{fig:topic_percentage} shows the order of the 19 topics based on the number of discussions per topic. Asking for opinion has the largest number of discussions. Developers also frequently query about troubleshooting, installation, and methodological aspects of developing and using fairness libraries. 


% \tbl\ref{tab:topic_source} shows the top sources of the detected topics. We see Fairlearn and AI Fairness 360 library being the top sources across the topics. That's because these two repositories contain the most number of issue discussions in our collected issue and issue comments dataset. 

% \begin{table}[h]
%   %\def\arraystretch{1.5}
%     \centering
%     \caption{Top sources of the detected topics}
%     \label{tab:topic_source}
%     \begin{tabular}{ll}
%     \toprule
%     \textbf{Topic}  										&	 \textbf{Top API Libraries}  \\ \midrule
% API expansion 	 	 & Fairlearn (67.7\%), AI Fairness 360 (16.1\%) \\ 
%  	 	 & Aequitas (6.5\%) \\ 
% \hline
% Artifact generation  	 	 & Fairlearn (86.6\%), AI Fairness 360 (6.1\%) \\ 
% and benchmarking 	 	 & BlackBoxAuditing (2.4\%) \\ 
% \hline
% Bias detection  	 	 & Fairlearn (63.6\%), Aequitas (16.4\%) \\ 
% metrics validation 	 	 & AI Fairness 360 (14.5\%) \\ 
% \hline
% Bias mitigation	 	 & Fairlearn (68.1\%), AI Fairness 360 (21.4\%) \\ 
% methodology 	 	 & EthicML (4.2\%) \\ 
% \hline
% Dataset usage 	 	 & Fairlearn (64.5\%), AI Fairness 360 (20.6\%) \\ 
%  	 	 & EthicML (9.3\%) \\ 
% \hline
% Dependency and Release 	 	 & Fairlearn (86.2\%), AI Fairness 360 (11.1\%) \\ 
%  	 	 & EthicML (1.8\%) \\ 
% \hline
% Documentation 	 	 & Fairlearn (91.9\%), AI Fairness 360 (4.7\%) \\ 
%  	 	 & EthicML (1.2\%) \\ 
% \hline
% Feature engineering  	 	 & Fairlearn (43.8\%), FairML (37.5\%) \\ 
% methodology 	 	 & AI Fairness 360 (6.2\%) \\ 
% \hline
% Fix warnings 	 	 & Fairlearn (66.7\%), AI Fairness 360 (22.2\%) \\ 
%  	 	 & Aequitas (11.1\%) \\ 
% \hline
% Installation and  	 	 & Fairlearn (53.3\%), AI Fairness 360 (29.9\%) \\ 
% shell commands 	 	 & Aequitas (6.0\%) \\ 
% \hline
% Metrics operation 	 	 & Fairlearn (91.8\%), EthicML (3.9\%) \\ 
%  	 	 & AI Fairness 360 (2.6\%) \\ 
% \hline
% Model development 	 	 & Fairlearn (91.7\%), AI Fairness 360 (4.2\%) \\ 
%  	 	 & EthicML (4.2\%) \\ 
% \hline
% Opinion 	 	 & Fairlearn (90.1\%), AI Fairness 360 (5.6\%) \\ 
%  	 	 & Aequitas (1.3\%) \\ 
% \hline
% Performance measurement 	 	 & Fairlearn (97.7\%), AI Fairness 360 (2.3\%) \\ 
% \hline
% Research 	 	 & Fairlearn (89.7\%), AI Fairness 360 (5.2\%) \\ 
%  	 	 & EthicML (3.1\%) \\ 
% \hline
% Testing 	 	 & Fairlearn (40.4\%), AI Fairness 360 (36.2\%) \\ 
%  	 	 & BlackBoxAuditing (8.5\%) \\ 
% \hline
% Troubleshooting 	 	 & Fairlearn (55.7\%), AI Fairness 360 (19.7\%) \\ 
%  	 	 & Aequitas (9.0\%) \\ 
% \hline
% UI 	 	 & Fairlearn (87.6\%), AI Fairness 360 (5.9\%) \\ 
%  	 	 & EthicML (3.5\%) \\ 
% \hline
% Understanding Fairness  	 	 & Fairlearn (91.8\%), AI Fairness 360 (4.1\%) \\ 
% Definition 	 	 & FairML (2.0\%) \\ 
% \hline
% \end{tabular}
% \end{table}

\begin{rqbox}{RQ4 Summary} 
We found 33 topics in the issue discussions of the 11 fairness API libraries. Our analysis reveals 
19 different kinds of issues that developers face while developing and using fairness libraries. 
These 19 topics are from all the six phases of the software development life cycle.
We observe that developers frequently face significant
methodological, troubleshooting, and installation issues while developing and
using fairness libraries. The issues cover all the stages of SDLC, although most
of the issues are related to Requirement, Deployment, and Maintenance.
Users need proper training on understanding what fairness is (especially in
a given context), what methodology to adopt, and how
to deal with these libraries. \rev{Our analysis, however, is limited to the issues posted and discussed within the libraries' own repositories only. We could not capture issues discussed outside these repositories; thus we may have missed other development challenges associated with these libraries.}   
\end{rqbox}



% \begin{rqbox}{RQ4 Summary} 
% We found 33 topics in the issue discussions of the 11 fairness APIs. Our analysis reveals 
% 19 different kinds of issues that developers face while developing and using fairness libraries. 
% These 19 topics are from all the six phases of software development life cycle.
% We observe that developers frequently ask for opinions, and face significant
% methodological, troubleshooting and installation issues, while developing and
% using fairness libraries. The issues cover all the stages of SDLC, although most
% of the issues are related to Requirement, Deployment, and Maintenance.
% Developers need proper training on understanding what fairness is (specially in
% a given context), and what methodology to adopt, and how
% to deal with these libraries. This observations present a call-to-arms to the educators for 
% developing more state-of-the-art curricula, which trains practitioners on dealing with fairness libraries at all the stages of  software development life cycle.
% \end{rqbox}

% \subsection{RQ5. Evolution of Topics}
% \gias{follow Section 4.2 of this paper for this RQ: \url{https://rdcu.be/cxhHV}}

% % \subsubsection{Motivation}
% We used topic modeling to find out the challenges that the developers are facing while developing the fairness API libraries. These topics and the categories we found have unique traits associated by the topic model. For example, the maintenance category pertains to the needs of understanding bug, and their fixes. 
% These needs may evolve over time and so do the the topics associated with each of these categories. In this research question we study this evolution to record and help the growing and changing fairness library development community and to identify any gaps that still need attention. 

% \subsubsection{Approach}
% In this research question we consider our six main categories of discussed challenge topics from the developers' perspective, as discussed on the issues and issue comments on the Github source code repository hosting website. Following previous study \cite{hanWhatProgrammersDiscuss2020}, we study the absolute and relative impacts of the topics identified in each category as follows.

% \nd\bf{Step 1. Topic Absolute Impact Computation.} We apply LDA topic for our corpus C and get K topics ($p_1$, $p_2$,........,$p_k$). The absolute impact metric for a topic $p_k$ in a month \ajoy{Shaiful vai, this will be quarter year/4 months as we didn't calculate it for a single month instead combined four months data together within a bin. So we need to update this formula. We can do that by denoting quarter year as q instead of using month m. Let me know whether this sound okay to you.} ($m$) can be defined as:
% \begin{equation}
% Impact_{absolute}(p_k;m) = \sum_{d_i=1}^{D(m)} \theta (d_i; p_k)   
% \label{eq:absoluteeq}
% \end{equation}
% Here, $\theta (d_i; t_k)$ denotes the possibility for a post ($d_i$) belonging to a topic $t_k$ and $D(m)$ is the total number of issue discussions in the month $m$.

% From the topic modeling we found 19 topics that we categorized into six higher level categories. We further refine this absolute-impact metric for a category $TC$ fir a month as:

% \begin{equation}
% Impact_{absolute}(TC_j;m) = \sum_{p_k}^{TC}Impact_{absolute}(p_k; m), 0 < j < TC
% \label{eq:absoluteeqcat}
% \end{equation}


% \nd\bf{Step 2. Topic Relative Impact Computation.}
% Relative impact metric signifies the proportion of the issue discussions for a particular topic ($p_k$) relative to all the discussions in our corpus ($C$) for a specific month ($m$). Following previous study \cite{hanWhatProgrammersDiscuss2020}, we compute the relative impact metrics for a topic ($p_k$) in a month ($m$) using the following formula:

% \begin{equation}
% Impact_{relative}(p_k,m) = \frac{1}{|D(m)|}\sum_{d_i=1}^\theta(d_i; p_k), 1\le i\le C 
% \label{relativeeq}
% \end{equation}

% Here, $\delta$ denotes the probability of a particular discussion ($d_i$) for the corpus ($C$ belonging to a specific topic ($p_k$) and $D(m)$ is the total number of posts in month $m$ that contain topic $p_k$.

% Following the absolute impact, for calculating the relative impact, we can refine the equation as follows where $TC$ denotes the top level topic categories and topic that belong to each of the topic category.

% \begin{equation}
% Impact_{relative}(TC;m) = \sum_{t_k}^{TC}Impact_{relative}(t_k;m)
% \label{relativeeqsw}
% \end{equation}

% \subsubsection{Results}
% Using the equations mentioned above we calculated the impacts of specific issue discussion topics and categories between year 2017 to 2022. 

% \nd\bf{Topic Absolute Impact}

% \begin{figure}[htb]
% \centering
% \includegraphics[scale=.5]{figs/analysis/topic_discussion_by_year.pdf}
% \caption{The evolution of overall issue discussions (issue body + comments) over time.}
% \label{fig:topic_discussion_by_year}
% \end{figure}

% \fig\ref{fig:topic_discussion_by_year} shows the evolution of overall issue discussions over time. This shows that the peaks of discussion occurred in Mid 2021. This also reveals that the issue discussion  has become increasingly popular from the starting of 2017. In this section we provide a mode in-depth explanation for the spikes of the curves.

% We show in \fig\ref{fig:topic_absolute_impact} the absolute impact of the topic categories. We can see that requirement analysis is the most discussed topic overall. We can see most of the topic category curves followed a similar trends, increased from 2017 to mid 2020, decreased for a moment, peaked at mid 2021 and decreased again.



% \nd\bf{Topic Relative Impact}

% In \fig\ref{fig:topic_relative_impact} we show the relative impact of the discussed topics. The initial portion of the curves (2017 to end of 2019) the curves fluctuated quite a bit, this may have been due to the smaller number of issue discussions that occurred with in this time period. However, after that time period we can see more stable trends. Topic categories such as Requirement analysis, Design increased at the end in popularity while the popularity of the rest of the topic categories (i.e., Development, Validation, Deployment, and Maintenance) decreased over time.

% \begin{rqbox}{RQ5 Summary} 
% The discussions are primarily associated to requirement analysis and designing phase during the implementation of fair machine learning models. This trends increases from 2017, with the popularity of bias API libraries. Over time, though the proportion of requirement analysis and design related discussions kept increasing relatively, the proportion of issue discussions kept dropping for the rest of the topic categories.
% \end{rqbox}
